SentiNet: Detecting Localized Universal Attacks Against Deep Learning Systems

SentiNet is a novel detection framework for localized universal attacks on neural networks. These attacks restrict adversarial noise to contiguous portions of an image and are reusable with different images -- constraints that prove useful for generating physically-realizable attacks. Unlike most other works on adversarial detection, SentiNet does not require training a model or preknowledge of an attack prior to detection. Our approach is appealing due to the large number of possible mechanisms and attack-vectors that an attack-specific defense would have to consider. By leveraging the neural network's susceptibility to attacks and by using techniques from model interpretability and object detection as detection mechanisms, SentiNet turns a weakness of a model into a strength. We demonstrate the effectiveness of SentiNet on three different attacks -- i.e., data poisoning attacks, trojaned networks, and adversarial patches (including physically realizable attacks) -- and show that our defense is able to achieve very competitive performance metrics for all three threats. Finally, we show that SentiNet is robust against strong adaptive adversaries, who build adversarial patches that specifically target the components of SentiNet's architecture.

==> Archive 2/abstract.tex <==
% !TeX root = ./main.tex
\begin{abstract}
\tool{} is a novel detection framework for \emph{localized universal attacks} on neural networks. These attacks restrict adversarial noise to contiguous portions of an image and are reusable with different images---constraints that prove useful for generating physically-realizable attacks.  Unlike most other works on adversarial detection, \tool{} does not require training a model or preknowledge of an attack prior to detection.  Our approach is appealing due to the large number of possible mechanisms and attack-vectors that an attack-specific defense would have to consider.  By leveraging the neural network's susceptibility to attacks and by using techniques from model interpretability and object detection as detection mechanisms, \tool{} turns a weakness of a model into a strength.  We demonstrate the effectiveness of \tool{} on three different attacks---i.e., data poisoning attacks, trojaned networks, and adversarial patches (including physically realizable attacks)---
%that have large variations in deployment mechanisms, 
and show that our defense is able to achieve very competitive performance metrics for all three threats. Finally, we show that \tool{} is robust against strong adaptive adversaries, who build adversarial patches that specifically target the components of \tool{}'s architecture.
\end{abstract}

==> Archive 2/adaptive_attack.tex <==
Adaptive Attacks:
A considerable number of defenses against adversarial attacks have been proposed only to be broken (cite) by 'adaptive attacks' that adapt to the presence of known defenses.  This has led to a cat-and-mouse game where defenses have to first discover and then account for new attacks constantly being introduced, creating an environment highly advantageous to adversaries.  Our proposed method diverges from this arms race by creating a generalizable defense that does not take the mechanism of an attack, which alleviates the need to tailor-design defenses towards specific attacks and provides the capability of detecting attacks that have not been seen before. We want to explore how robust our method is against adaptive attacks by attempting to compromise each component of our defense.



Threat Model:
	1. Localized universal adversarial patch
		a. Our threat model deals with over-the-air attacks, where you can't just attack a digital image
		b. A sufficiently large image can override any image, as described in "Adversarial Patches" - must be small
		c. Attacks are generally 'universal' - attacks cannot be specific to a specific image in an over-the-air setting, must be robust to viewpoint, resolution, and brightness changes
	2. Our defense assumes - attacks are small, and attacks misguide towards a certain class
		a. Our defense uses GradCam+FRCNN to segment out the small patch
		b. Overlays suspected attack onto other test set I' to get number of misguided (2) and also overlays noise onto test set l' to get the confidence value after noising (1)
		c. Normal images either have high (1) and low (2) (associated with small patches), high (2) and low (1) (associated with large patches), or low (1) and low (2) (large patches of useless information).  Only adversarial images will have high (1) and low (1).
		
	3. Proposed Attack - Thresholding
		a. We do not share I' with any outside parties, which means the attacker cannot manipulate the behavior on I' for either (1) or (2).  The attacker cannot attack the thresholding behavior.
	4. Proposed Attack - Fast RCNN
		a. Fast RCNN consists of two parts - the original network and selective search
		b. Overall, Fast RCNN is used to narrow down our GradCAM mask, so attacking it will only slighly decrease the accuracy of our defense rather than subveting it.
		c. Because we use the original network for classification, if our original network is susceptible, the network used for RCNN will also be susceptible; therefore it is impossible to bypass the bounding box classification network.
		d. Attacking selective search is very difficult due to the exhaustive properties of selective search - selective search is not a gradient descent based technique meaning its hard to construct an adversarial attack; it is based detecting edges and color changes to create many object proposals. Therefore, it is impossible to prevent the bounding boxes from being proposed outside of the patch
	5. Proposed Attack - Multiple Patches
		a. First Attack - disjoint attacks targeting same classes -  our experiment shows this doesn't work
		b. Second Attack - single patch targeting different classes - detect patch + object as the natural object will bypass the FastRCNN eliminations - if more than 3 objects in the same area - reject 
		c. Third Attack -detect patch+object as 1 object - lots of disjoint attacks will bypass the FastRCNN eliminations; we can increase the number of FastRCNN proposals, increasing by linear runtime. 
	6. Proposed Attack - GradCAM
		a. A possible subversion for GradCAM is to make the GradCam activate outside of the patch, either making the mask segment too much of the image out or to miss detecting the patch altogether.  Our experiments show that it is possible to perturb an entire image to create a certain GradCAM output, but it is impossible to affect the GradCAM outputs outside of a localized patch
Another possible attack is to minimize the amount the patch shows up on GradCAM.  We first show that adding perturbed noise to minimize the patch will decrease the effectiveness of the attack.  We show that this is the case even with joint training (show the curve).  We believe this is evidence that that it is impossible to optimize for both minimizing GradCAM and the attack behavior

==> Archive 2/approach.tex <==
% !TeX root = ./main.tex
\begin{figure*}[!htbp]
    \centering
    \includegraphics[width=1\textwidth]{figures/approach.pdf}
    \caption{Overview of the \tool{} architecture to protect a model $f_m$.  The output and class proposals of an input are used to generate masks and image tests, which are then fed back into $f_m$ to generate values for boundary analysis and attack classification.}
    \label{fig:approach_overview}
\end{figure*}

\section{\tool}
\label{sec:sentinet}

In this section, we present \tool{}. The goal of \tool{} is to identify adversarial inputs that will hijack the prediction of the neural network without assuming the knowledge of the attack vector beforehand, e.g., exploiting vulnerabilities of compromised and uncompromised networks. The core insight of \tool{} is to use the very behavior of adversarial misclassification to detect an attack. 

The architecture of \tool{} is shown in \Cref{fig:approach_overview}. First, \tool{} uses techniques from model interpretability and object detection to extract from an input scene $x$ those regions that most highly influence the model prediction $y$ (\Cref{sec:attack_localization}). These regions likely contain the malicious object (if present) as well as benign salient regions. Then, \tool{} applies these extracted regions on a set of benign test inputs and observes the behavior of the model. Finally, \tool{} compares the synthetic behaviors with the known behavior of the model on benign inputs, to detect prediction hijacking (\Cref{sec:fuzzing}). 


\subsection{Adversarial Object Localization}
\label{sec:attack_localization}

The first phase of our approach intends to localize on the given input the regions that might contain malicious objects. The idea is to identify the parts of the input $x$ that contribute to the model prediction $y$. Because the attack is small and localized,  we can hope to recover the true class of input $x$ if we evaluate the model on a segmented input that contains no part of the attack. In the following, we look into the details of this phase. First, we present a segmentation-based approach to propose classes (see \Cref{fig:approach_overview}.a). Then, starting from proposed classes and the given input, we generate a mask for $x$ that may contain the malicious object (see \Cref{fig:approach_overview}.b).

\subsubsection{Class Proposal via Segmentation}%\label{sec:class_proposal}
The detection of the attack begins with the identification of a set of possible classes that may be predicted by the model $f_m$. The first of such classes is the actual prediction, i.e., $y = f_m(x)$. The other classes are identified by segmenting the input $x$ and then evaluating the network on each segment. \Cref{alg:class_proposal} shows the algorithm to propose classes via input segmentation. 
Different approaches can be used to segment a given input $x$ including sliding windows and network-based region proposals~\cite{ren2015fasterrcnn}.
% \GP{@Edward: please add example of type 1} and \GP{@Edward: please add example of type 2}. 
In our approach, we use the selective search image segmentation algorithm~\cite{uijlings2013selectivesearch}. Selective search generates an exhaustive list of region proposals based on the patterns and edges found in natural scenes~\cite{uijlings2013selectivesearch}. Then, we evaluate each proposed segment, i.e., $f(x_p)$, and return the $k$ most confident predictions, where $k$ is a configuration parameter of \tool{}.  We exclude the primary class $y=f_m(x)$ from our choice of $k$ classes.
A general guideline towards selecting $k$ is to set it to be slightly higher than the amount of classes that are present in the dataset per-image.  
In our case, Imagenet~\cite{deng09imagenet} has around 1.5 classes per image, and we set $k$ to 2.
% \GP{explain that we have a primary class $y=f_m(x)$ and $C$ are only secondary ones.}

% \spreview{Unclear how $k$ is selected in practice
% Worth showing - try with 2, 3, 4}


\begin{algorithm}
    \footnotesize
    \Input{$f_m$ -- model\;
    ~~~~~~$x$ -- input of $f_m$\;
    ~~~~~~$y$ -- primary class, i.e., $y=f_m(x)$\;
    ~~~~~~$k$ -- propositions}
    \Output{$C$ - set of proposed classes and confidence ($|C|=k$)}

    $P$ = \SelectiveSearch{$x$}\;
    $C$ = $\{(y_p, conf_p): \forall x_{p} \in P, (y_p, conf_p) = f_m(x_{p})\wedge y_p \neq y\}$\;
    $C$ = \TopConf{$C$, $k$}\;
    \Return{$C$}

    \caption{ClassProposal}
    \label{alg:class_proposal}
\end{algorithm}

\subsubsection{Mask Generation}%\label{sec:class_proposal}
Once the class proposal C is obtained, the second step of \tool{} consists of identifying the regions of $x$ that most highly influence the predictions C. To find these regions, we resort to techniques to explain and interpret model predictions. 

%One strategy attempts to ``quantify'' the relevance of individual pixels of the input, e.g., using saliency maps~\cite{yosinski2015deepvis}. While effective in practice, focusing on individual pixels may result in a mask of non-contiguous pixels. Sparse masks may miss elements of the malicious object and are not suitable for the model testing phase (see~\Cref{sec:fuzzing}). Alternative approaches do not operate on individual pixels but attempt to recover discriminative image regions used by the model to identify the inputs of the same class. Unfortunately, many of these approaches require modifying and fine-tuning a base model, e.g., Class Activation Mapping (CAM)~\cite{zhou2015cam}. Such modifications may alter the behavior of the model, including the malicious behavior that \tool{} intends to detect.\footnote{We verified that CAM cannot be used with trojaned network as it removes the last layer (i.e., Layer FC6-8 of face recognition model of~\cite{Liu2018TrojaningAO}) rendering the trigger trojan undetectable.}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figures/imagenet.png}
%     \includegraphics[width=0.48\columnwidth]{figures/gradcam_vis.png}
%     \caption{Example of heatmap created with Grad-CAM over the original input using the model prediction. Red and yellow regions are for \FIXME{continue}. The left-hand side shows a malicious input. The right-hand side shows a benign input picture.\GP{@Edward: Please remove white margin of the picture and enlarge it.}}
%     \label{fig:class_proposal}
% \end{figure}

A particularly suitable approach for our goal is Grad-CAM~\cite{chattopadhyay2017gradcamplus}, a model-interpretation technique that identifies contiguous spatial regions of an input without requiring modifications to the original model. At a high level, Grad-CAM uses gradients computed in the final layers of a network to calculate the saliency of input regions. For class $c$, Grad-CAM calculates the gradients of the model's output $y^c$ (the model's \emph{logit} score for class $c$) with respect to each of the $k$ feature maps $A^k$ of the model's final pooling layer to obtain $\frac{\delta y^c}{\delta A^k}$. The mean gradient value of each filter map, or ``neuron importance weight'', is denoted $\alpha_c^{k} \coloneqq \frac{1}{Z} \Sigma_i \Sigma_j \frac{\delta y^c}{\delta A^k}$. Finally, the feature maps $A^k$ are weighted by their neuron importance and aggregated to obtain the final Grad-CAM output: $L^c_{Grad-CAM} \coloneqq ReLU(\Sigma_k \alpha_c^{k} A^k)$. Here, $ReLU(x)=\max(x, 0)$ is the ReLU activation function~\cite{glorot2011deeprelu} which retains only the positive gradient signals for class $c$. The output of Grad-CAM is a coarse heatmap of the positive importance of the image, usually at a lower resolution that the input image due to downsampling in the model's convolutional and pooling layers. Finally, masks are produced by binarizing the heatmap with a threshold of 15\% of max intensity.  We use this mask to segment salient regions for the next steps.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\columnwidth]{figures/object_detector.png}
%     \includegraphics[width=0.48\columnwidth]{figures/object_detector_face.png}
%     \caption{Visual example of the selective search segmentation approach. The left-hand side is an image with a malicious object. The right-hand side is a benign input image. \GP{@Edward: Please remove white margin of the picture and enlarge it.}\GP{Add two examples of selective search on two images of our experiments}}
%     \label{fig:selective_search}
% \end{figure}


% \begin{figure}[htbp]
%     \centering
% \includegraphics[width=0.32\columnwidth]{figures/face_square_heatmap_toolarge.png}
% \includegraphics[width=0.32\columnwidth]{figures/face_mask_toolarge.png}
%     \caption{Example of region extraction when using only one Grad-CAM mask. The left-hand side shows the Grad-CAM heatmap of the trigger trojan. The right-hand side the extracted region.}
%     \label{fig:region_refinement}
% \end{figure}

%\GP{@Edward: Please remove white margin of the picture and enlarge it.}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.32\columnwidth]{figures/face_square_heatmap_toolarge.png}
% \includegraphics[width=0.32\columnwidth]{figures/face_mask_toolarge.png}\\ \vspace{0.2cm}
% \includegraphics[width=0.32\columnwidth]{figures/face_square_heatmap_toolarge.png}
% \includegraphics[width=0.32\columnwidth]{figures/face_square_354.png}
% \includegraphics[width=0.32\columnwidth]{figures/face_bettermask.png}
%     \caption{Top Row: Example of region extraction when using only one Grad-CAM mask. The left-hand side shows the Grad-CAM heatmap of the trigger trojan. The right-hand side the extracted region.  Bottom Row: Combining masks of class proposals increases the precision of the region containing the adversarial object.\FT{Give slightly more detail here: The left is a GRADCAM with respect to the targeted class, the middle is a GRADCAM with respect to the true class.}}
%     \label{fig:precise_mask}
% \end{figure}

\begin{figure}[ht]
    \centering
	\begin{subfigure}[b]{1\columnwidth}
        \includegraphics[width=1\columnwidth]{figures/mask_reduction_top.pdf}
        \caption{}
    \end{subfigure}
    
	\begin{subfigure}[b]{1\columnwidth}
        \includegraphics[width=1\columnwidth]{figures/mask_reduction_bottom.pdf}
        \caption{}
    \end{subfigure}
    \caption{Differential mask generation to remove ambiguous areas. \textbf{(a)} Example of Grad-CAM mask using prediction $y$ covering benign areas. \textbf{(b)} Example of precise mask by removing masks of class proposals $C$.}
    \label{fig:precise_mask}
\end{figure}

% \FT{Give slightly more detail here: The left is a GRADCAM with respect to the targeted class, the middle is a GRADCAM with respect to the true class.}

% \GP{@Edward, can we merge Fig.4 and Fig.5 in a single group of figures to show how we improve mask precision?}

% \GP{@Edward: Please remove white margin of the picture and enlarge it.}

We generate masks with Grad-CAM as shown in \Cref{alg:mask_generation}. We start by extracting the mask using Grad-CAM for the input $x$ and prediction $y$. As Grad-CAM can identify salient areas for benign classes, the resulting mask may span over both benign and malicious regions. An illustrative example is in \Cref{fig:precise_mask}, where the Grad-CAM generated heatmap for a facial recognition network covers both a trojan trigger patch but also the original face. To improve the accuracy of the mask, we also extract a mask for each proposed class $y_{p}$. Then, we use these additional heatmaps to generate secondary masks to improve the original mask for the prediction $y$ by subtracting common regions. This results in a set of masks that highlight only the localized attack and not the other salient regions in the image. 

%\vspace{0.2cm}\noindent\textbf{Precise Mask Generation}---%\label{sec:malicious_region} 
%\GP{Can we simplify this part and merge it with the Mark Generation?}
% Although Grad-CAM can successfully identify discriminative input regions corresponding to adversarial objects, it may also identify benign salient areas. An illustrative example is in \Cref{fig:precise_mask}, where the Grad-CAM generated heatmap for a facial recognition network covers both a trojan trigger patch but also the original face. To improve the accuracy of the mask, we query the model for additional predictions on selected regions of the input image. Then, for each prediction, we use Grad-CAM to extract a mask for the input area most relevant for the prediction. Finally, we combine these additional masks to refine the mask of the initial prediction $y$. 

% Once we derive a list of possible classes present in the picture, we carve out the regions of $x$ more relevant for each predicted class. For simplicity, in this section, we assume that each input can contain only one malicious object. We show how to generalize this approach to multiple malicious inputs in \Cref{sec:adaptive_attacks}. \Cref{alg:mask_generation} shows the procedure to extract input regions from $x$. 

% We start by extracting the mask using Grad-CAM for the input $x$ and prediction $y$. We also extract a mask for each proposed class $y_{p}$. Performing Grad-CAM on the other proposed classes allows us to locate the important regions of the image besides the adversarial attack. Additionally, because the adversarial region is often negatively correlated with the non-targeted classes, the heatmap actively avoids highlighting the adversarial regions of the image.  
% We can use these heatmaps to generate secondary masks to improve our original mask by subtracting regions where the masks overlap. This results in masks that highlight only the localized attack and not the other salient regions in the image.  In \Cref{fig:precise_mask}, we can see this approach applied to generate a more precise mask containing mostly the adversarial region only.

% \spreview{One could also consider groups of segments (pairs, triples, etc.) when producing these proposals. While this increases the time complexity combinatorially, it could result in better accuracy. What was the rationale for classification individual segments?: We can say instead of combinatorially, we do it iteratively}


\begin{algorithm}
    \footnotesize
    \Input{$f_m$ -- model\;
    ~~~~~~$x$ -- input for $f_m$\;
    ~~~~~~$y$, $conf$ -- model prediction on $x$\;
    ~~~~~~$C$ -- proposed classes}
    \Output{$M$ - masks for candidate regions with the malicious object}

    $mask_y$ = \MaskGradCAM{$f_m$, $x$, $y$}\;
    $M$ = $\{ (mask_y-$\MaskGradCAM{$f_m$, $x$, $y_{p}$}$, conf_{p})$ 
            $: (y_{p}, conf_{p}) \in C \}$\;
    %$R$ = $\{ x * mask : mask \in C\}$\;
    \Return{$\{mask_y\} \cup M $}

    \caption{MaskGeneration}
    \label{alg:mask_generation}
\end{algorithm}

\subsection{Attack Detection}
\label{sec:fuzzing}

Once we identified regions $M$ of the inputs $x$ that may be containing malicious inputs, we test the model $f_m$ to determine whether any of the regions can hijack the expected predictions of a set of benign test inputs. 

% The detection of an attack requires two steps. First, as described above, \tool{} extracts input regions that are likely to contain adversarial patches. Then, \tool{} \emph{tests} each of these regions on a set of benign images, as detailed below, to discriminate adversarial regions from benign ones.

\subsubsection{Test Generation} Once an input region is localized, \tool{} observes the effects the region has on the model to determine whether the region is adversarial or benign. To do so, \tool{} overlays the suspected region on a set of benign test images $X$, which are often shipped together with deployed models. Test images $X$ are fed back into the network, where the number of fooled examples are counted and used for adversarial images. Intuitively, the higher the number of mutated images can fool the model, the more likely the suspected region is an adversarial attack.

% \spreview{The overlay operation seems to apply the mask in the same position and the same orientation as in the original image. Why not consider different positions and locations?
% Clarify - might not work as a patch after moving
%}

When the recovered region is small, this technique is effective at distinguishing adversarial and benign inputs, as small benign objects cannot typically overwhelm a network’s prediction. However, one problem of this approach is that a region (whether adversarial or benign) that covers a larger fraction of the input image will likely cause misclassifications when overlaid onto most other images because they occlude the original object.

To measure the extent to which an overlaid region causes misclassifications simply by occluding the original object, rather than by virtue of highly-salient features, we perform a second test where we replace the content of the overlaid region with an inert pattern of low saliency (e.g., Gaussian noise). We expect that adversarial regions will cause many misclassifications when overlaid on the test set, but have little effect on the network when replaced by an inert pattern before being overlaid. In contrast, we expect benign patterns to either cause few misclassifications, or to occlude objects and thus also disrupt the model when replaced by inert patterns. Algorithm~\ref{alg:testing} shows the algorithm we use to test extracted regions. For each region, we check how many overlaid test images fooled the network, and how confident the model is when classifying images overlaid with inert patterns.

\begin{algorithm}

    \Input{$f_m$ -- model\;
    ~~~~~~$x$ -- input for $f_m$\;
    ~~~~~~$y$ -- class of $x$\;
    ~~~~~~$M$ -- proposed masks\;
    ~~~~~~$X$ -- bening test images\;}
    \Output{$Fooled$, $AvgConf$}

    $R$ = $\{ x * mask : mask \in M\}$\;
    $IP$ = \InertPattern($M$)\;
   
    $X_{R}$ = \Overlay($X$, $R$)\;
    $X_{IP}$ = \Overlay($X$, $IP$)\;

    $fooled_{y_R}$ = $0$, $avg_{{conf}_{IP}}$ = $0$\;

    \For{$x_{R}$,$x_{IP} \in X_{R}, X_{IP}$}{
        $(y_R, conf_R), (y_{IP}, conf_{IP})$ = $f(x_{R}), f(x_{IP})$\;

        \If{$y_R == y$}{
            $fooled_{y_R}$ += 1
        }
        
        $avg_{{conf}_{IP}}$ += $conf_{IP}$
    }
    $avg_{{conf}_{IP}}$ = $\frac{avg_{{conf}_{IP}}}{|X|}$\;
    
    \Return $fooled_{y_R}$, $avg_{{conf}_{IP}}$\;
    \caption{Testing}
    \label{alg:testing}
\end{algorithm}

\subsubsection{Decision Boundary for Detection} 

With these two met- rics (number of images fooled and average inert pattern confidence values) we can determine whether an input x is adversarial. A naive approach is to use thresholding based rules, but it is hard to determine how to set the thresholds and which metric holds more importance. Instead, we use metrics collected on clean examples to train a simple two-feature one- class classifier and classify outliers as adversarial.

We examine this problem by plotting metrics from an example task in a 2D plot in Figure \ref{fig:example_boundary detection}, where the red triangular dots represent adversarial examples and the blue circular dots represent clean examples. We observe that the adversarial and clean points can be easily separated using a parabolic function, suggesting that a classifier approach such as linear regression or support vector machine could be used. However, this would operate under the false assumption that we have prior examples of adversarial inputs. Ideally, we want to create a technique that would allow us to identify an unseen adversarial input as an attack based on the attack-agnostic metrics.

% \GP{@Edward: Where are these red dots?}
% \GP{@Edward: please add a reference to the paper.}

We notice a general pattern where adversarial examples are usually clustered near the top-right of the plot.  Because adversarial examples are designed to cause misclassifications when applied to other images and not overly obstruct the other important regions of an image, it makes sense that both the number of images fooled and the average noisy confidence metrics of an adversarial example would be high. We can use our set of benign test images to generate statistics of the metrics of normal examples, which will then allow us to formulate when an input is abnormally adversarial.

We can use our collected metrics on clean examples to approximate a curve. By taking the points most likely to be the bounds of the statistics of our examples, we can approximate a curve where points lying outside our curve function can be classified as attacks. We collect our points by taking the points with the highest y-values for x-intervals, and then using a non-linear least squares function to approximate our curve. We then use our approximated curve to set classify attacks by calculating the distance between a curve and a point ---using the Constrained Optimization by Linear Approximation (COBYLA) method~\cite{conn1997cobyla}---and determining whether that distance is within a threshold estimated by the distances of clean examples lying outside the curve.

\begin{algorithm}[ht]
   
    \Input{$B$ -- sampled behavior of $f_m$}
    \Output{$f_{curve}$ -- approximated curve function\; 
    ~~~~~~~$d$ -- acceptable distance from $f_{curve}$}

    $f_{curve}$ = \ApproximateCurve{\OutPts{$B$}}\;
    
    $avg_d$ = $0$\;
    \For{$(x, y) \in B$}{
        \If{$f_{curve}(x) > y$}{ 
            $avg_d$ += \COBYLA{$(y, x), f_{curve}$}\;
        }
    } 
    $d$ = $\frac{avg_d}{|B|}$\;
    \Return{$f_{curve}$, $d$}\;

    \caption{DecisionBoundary}
    \label{alg:decision_boundary}
\end{algorithm}

\begin{figure}[ht]
        \centering
        \includegraphics[width=1.0\columnwidth]{sentinet_figs/face_400_curvefit.png}
        \caption{Example of boundary detection for the trojaned experiments using 400 data points and random noise as inert pattern.  On the left, the adversarial and benign metrics are plotted as red triangles and blue circles respectively; on the right, we plot the curve proposal from the sampled points, i.e., the benign test images $X$.}
    \label{fig:example_boundary detection}
\end{figure}

%\GP{increase the font size of the axis.} 

% \begin{figure}
%     \centering
% \includegraphics[width=0.475\columnwidth]{sentinet_figs/face_400_nocurve.png}
% \includegraphics[width=0.475\columnwidth]{sentinet_figs/face_400_curvefit.png}
%     \caption{Example of boundary detection for the a trojaned using 400 data points and random noise as inert pattern.  On the left, the adversarial and benign metrics are plotted as red triangles and blue circles respectively; on the right, we plot the curve proposal from the sampled points, i.e., the benign test images $X$.\GP{increase the font size of the axis.} }
%     \label{fig:example_boundary detection}
% \end{figure}

==> Archive 2/background.tex <==
% !TeX root = ./main.tex
\section{Background}
\label{sec:background}

% Before presenting our approach, we introduce the building blocks of this paper. We start with the fundamental concept of neural networks (\Cref{sec:neural_networks}) and their integration in deep learning systems (\Cref{sec:dl_systems}). Then, we present the security threats and possible attacks against DL systems (\Cref{sec:threat_model}). Next, in \Cref{sec:discussion}, we discuss results and features of our approach. Finally, in \Cref{sec:related_work}, we present related works and in \Cref{sec:conclusion} the conclusion.

% \subsection{Neural Networks} 
% \label{sec:neural_networks}

\subsection{Deep Learning Systems}
\label{sec:dl_systems}

% \begin{figure}
% 	\centering
% 	\begin{subfigure}[b]{1\columnwidth}
% 	\includegraphics[width=1\columnwidth]{figures/dl_system_overview.pdf}
% 	%\caption{}
% 	%\label{fig:dl_system}
% 	\end{subfigure}
% 	% \begin{subfigure}[b]{1\columnwidth}
% 	% \includegraphics[width=1\columnwidth]{figures/dl_system_threat_model.pdf}
% 	% \caption{}
% 	% \label{fig:dl_system_threat}
% 	% \end{subfigure}
%     % \caption{DL system and threat model overview. \textbf{(a)} An example of DL system processing a stream of sensor data to perform an action. \textbf{(b)} The threats to DL systems are malicious scene objects and compromised models.\GP{Figure 1 [...] sets a misleading expectation that the paper will consider the full end-to-end attack including the actuator.}}
%     \caption{Example of DL system processing a stream of sensor data to perform an action.}
%     \label{fig:dl_system}
% 	\label{fig:dl_system_overview}
% \end{figure}

\emph{Deep learning} (DL) is a branch of machine learning which focuses on multi-layered artificial neural networks~\cite{lecun2015deep}. A neural network can be defined as a standard machine learning function $f_m$, which given an input $x$ returns a prediction $y$ and prediction-confidence $conf$; i.e. $(y, conf)=f_m(x)$.  Convolutional Neural Networks (CNN)~\cite{lecun1995convolutional} are a specific architecture of neural network primarily targeted at computer vision tasks. Common CNN architectures include VGG-16~\cite{simonyan2018vgg16}, ResNets~\cite{he2015resnet} and Inception models~\cite{szegedy2014inception}.

% \subsection{Deep Learning Systems}
% \label{sec:dl_systems}


\emph{DL systems} are computer systems that rely on neural networks to perform specific tasks. At its essence, a DL system takes in an input, computes an output value, and makes a prediction based on the output. The analysis performed by a DL system is often a classification task such as a face-based user authentication mechanisms, voice recognition, or voice-to-text system. Recently, DL systems have been proposed for autonomous vehicles and digital assistants~\cite{zhang2018dlreview}.

% \FIXME{Find example 1}, \FIXME{Find example 2}, and \FIXME{Find example 3}.

% In this paper, we focus on DL systems that feed a neural network with sensor data. The prediction of the neural network is used to determine an appropriate action. \Cref{fig:dl_system} shows an example of a DL system implementing a face recognition system to unlock a mobile device or to let a user into a building. The scene includes the user's face and other background objects. The sensor can be a CCD sensor of a camera that returns a digital image of the scene. The image is processed by a face classifier which predicts the user identity. If the user identity is valid, the actuator will unlock the device or open the gate.



% \GP{Present \Cref{fig:dl_system_overview}. Present a DL system that process over-the-air inputs. Present the sensors for the analog-to-digital conversion. Say that DL systems use pre-trained models. Say that pre-trained models can be used either as-is, or they can be transformed (stripped off the classifier). These models are trained by someone else. The developers of a DL system do fine-tuning to adjust the model to the new task. Re-using existing models is an emerging trend. For instance, it has been estimated that 13.7\% of ML systems on GitHub uses one popular model~\cite{ji2018model}.}

\subsection{Threat Model}
\label{sec:threat_model}

In this work, we assume a scenario where a DL system uses a pre-trained deep CNN model to classify sensor data. Within this scenario, the goal of the adversary is to hijack the prediction of the model by providing a malicious image to the CNN model. In \Cref{sec:lua}, we present the properties of the malicious inputs considered in this paper, and in \Cref{sec:attack_vectors}, we present existing techniques to mount the attacks. Additionally, we assume an adversary that is aware of the defense mechanisms, and that can generate malicious images to bypass \tool{}. In \Cref{sec:lua}, we present such an adversary.

\begin{figure*}
	\centering
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.45\columnwidth]{figures/trojan_cropped.png}
        \includegraphics[width=0.45\columnwidth]{figures/example_trojan_face.jpg}
        \caption{Trojan trigger.}
        \label{fig:trigger}
    \end{subfigure}\hfill
    \vspace{0.2cm}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.45\columnwidth]{figures/flower_nobg.png}
        \includegraphics[width=0.45\columnwidth]{figures/example_stopsign.png}
        \caption{Backdoor.}
        \label{fig:backdoor}
    \end{subfigure}\hfill
    \vspace{0.2cm}
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=0.45\columnwidth]{figures/adversarial_patch.png}
        \includegraphics[width=0.45\columnwidth]{figures/banana_table_patch.jpg}
        \caption{Adversarial patch.}
        \label{fig:adv_patch}
	\end{subfigure}
    \caption{Examples of localized universal attacks. (a) Trojan trigger for trojaned VGG-16 model for face recognition~\cite{Liu2018TrojaningAO}. (b) Backdoor for poisoned Faster-RCCN for road signs detection~\cite{gu2017badnets}. (c) Adversarial patch for uncompromised VGG-16 for ImageNet~\cite{brown2017adversarialpatch}.}
    \label{fig:lua}
\end{figure*}

\subsubsection{Localized Universal Attacks}
\label{sec:lua}

The goal of the adversary is to hijack the prediction of the model to gain control of the actions performed by the DL system. To achieve this goal, the adversary can craft a malicious object and place it in the input image, e.g., inside the visual scene of the sensors. The malicious objects considered in this paper are \emph{localized}, i.e., the object is constrained to a small contiguous region of the image. The objects of this paper are also \emph{universal}, i.e., the object is created once and reused many times with different input images. \Cref{fig:lua} shows three examples of universal, localized malicious objects. 

\subsubsection{Attack Vectors}
\label{sec:attack_vectors}

The adversary can construct and use malicious objects in different ways, that we review in this section. For example, the adversary can ``alter'' the behavior of the network to respond to a malicious object before its deployment in a DL system. Examples of these attacks are trojaning~\cite{ji2018model, Liu2018TrojaningAO} or poisoning attacks~\cite{gu2017badnets}. Alternatively, the adversary can also cause misclassifications to uncompromised models by crafting ad-hoc malicious object, e.g., adversarial patches~\cite{sharif2016glasses,kurakin2016adversarial, brown2017adversarialpatch,evtimov2017robust,eykholt2018physical,athalye2017synthesizing}. 



% In this paper, we consider three known techniques, i.e., adversarial patches~\cite{sharif2016glasses,kurakin2016adversarial, brown2017adversarialpatch,evtimov2017robust,eykholt2018physical,athalye2017synthesizing}, data poisoning attacks~\cite{gu2017badnets}, and model trojaning attacks~\cite{ji2018model, Liu2018TrojaningAO}. Furthermore, we consider an adversary that is aware of the mechanism and the architecture of defense to protect a DL system. Such an attacker can generate malicious objects with the goal of bypassing or attacking internal components of our defense.

\paragraph{Compromised Models} One way to mount localized universal attacks is to compromise the network before deployment, by establishing a strong response between a class and a malicious object. Over the past few years, two attack vectors have emerged, i.e., data poisoning attacks and trojaning attacks. In a data poisoning attack, the adversary compromises the network at training time by inserting malicious inputs, i.e., benign images with malicious objects called \emph{backdoors} (see \Cref{fig:backdoor}), in the training set~\cite{gu2017badnets}. In a model trojaning attack, the adversary compromises the network by modifying the weights of selected neurons to respond to a specific \emph{trojan trigger}~\cite{ji2018model, Liu2018TrojaningAO} (see \Cref{fig:trigger}).

% Training a large neural network from scratch requires a huge amount of data and computation, and developers tend to reuse pre-trained networks~\cite{bengio2012deep} readily available on online repositories such as Model Zoo\footnote{See \url{https://modelzoo.co/}}. Reusing a pre-trained neural network exposes a DL system to several attacks. In particular, we consider two attacks that originate when the origin of the model is untrusted. One method to compromise a neural network is via \emph{data poisoning attacks}. In a data poisoning attack, the adversary inserts malicious inputs, i.e., \emph{backdoors} to compromise the model during training~\cite{gu2017badnets}. Instead of training a model with malicious data points, the adversary could also \emph{trojan} a neural network by modifying the weights of selected neurons~\cite{ji2018model, Liu2018TrojaningAO} to respond to a specific \emph{trigger}. For both trojaned and poisoned networks, the adversary can modify a network to respond to specific objects.

\paragraph{Vulnerabilities of Uncompromised Models} Even if the networks are integrity protected, an adversary can hijack models' predictions by exploiting the inherent instability of neural networks when processing maliciously-crafted inputs. Recent works have shown that adversaries can create localized universal malicious objects, e.g., printed patches~\cite{sharif2016glasses,brown2017adversarialpatch,eykholt2018physical,evtimov2017robust} or 3D objects~\cite{athalye2017synthesizing} (see, e.g., \Cref{fig:adv_patch}), that can fool a model under real-world conditions such as lighting, sensor noise, and rotation.

% To mitigate the risks of compromised models, developers can resort to trusted third parties to train and deliver an ad-hod model. Unfortunately, as pointed out by prior works, models are inherently unstable when processing maliciously-crafted inputs, i.e., \emph{adversarial examples}~\cite{szegedy2013boxlbfgs,goodfellow2014fgsm}, that can be used to hijack the model prediction. Most of the existing literature on adversarial examples requires the attacker to control the neural network input at the byte level. In a physical DL system, this means that the attacker controls either the sensor to generate the desired stream of bytes or the communication channel between the sensor and the model to modify the data. However, the sensor and the communication channel of a DL system may not be accessible by an attacker. As a result, the attacker can only influence the stream of data values to the model by showing the sensor physical objects. Recent works have shown that adversaries can create malicious physical objects, e.g., printed patches~\cite{sharif2016glasses,brown2017adversarialpatch,eykholt2018physical,evtimov2017robust} or 3D objects~\cite{athalye2017synthesizing}, that can fool a model under real-world conditions such as lighting, sensor noise, and rotation. As opposed to the more traditional perturbations, physical perturbations are \emph{localized} in a \emph{small} region of the input.


\subsubsection{Adaptive Adversary} Over the past years, many ideas have been proposed to protect neural networks from attacks. While some new ideas have moderately increased the robustness of neural networks (e.g., strong adversarial training~\cite{madry2018towards}), many do not adequately protect networks against adversaries aware of the specific defense mechanism being used (see, e.g.,~\cite{carlini2017adversarial,athalye2018obfuscated,tramer2020adaptive}). Accordingly, in this paper, we assume a strong white-box adversary that is fully aware of \tool{}, its architecture and mechanisms. 

%For example, such an adversary may attempt to generate an adversarial object that will be able to fool both the model and the components of \tool{} meant to protect the network. Also, we assume that the adversary does not know the configuration of a specific instance of \tool{}, i.e., the benign test set $X$ and the inert pattern---two key parameters essential to the detection of malicious objects that we introduce in \Cref{sec:sentinet}.

% \GP{Explain that we focus on attackers with a specific goal, i.e., they want to misuse the DL system in specific way. They do not intend to cause random errors.}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[height=1in]{figures/banana_table_patch.jpg}
%     \includegraphics[height=1in]{figures/example_trojan_face.jpg}
%     \includegraphics[height=1in]{figures/example_stopsign.png}
%     \caption{Examples of Physical Attacks.  From left to right: an Adversarial Patch~\cite{brown2017adversarialpatch}, a Trojaning Trigger~\cite{Liu2018TrojaningAO}, and a Backdoor~\cite{gu2017badnets}.  These attacks represent the diversity of the current attack literature.}
%     \label{fig:pull_figure}
% \end{figure}

%\subsection{Attacks to Neural Networks}

% \subsubsection{Poisoning Attacks}
% An attacker with control of the training phase of a model can create inherent biases in the model by mislabelling data~\cite{shafahi2018poisonfrog}.  One approach would be to make a model susceptible to a particular pattern that will always lead to a certain output.  When the pattern is not present, the model will behave normally, making such attacks difficult to detect or anticipate.

% An example can be found in Badnets~\cite{gu2017badnets}, which a pattern imposed on objects to poison the data, retraining the model on faulty labels.  
% In this particular setting, the attack is demonstrated on an object detection network~\cite{ren2015fasterrcnn} on a traffic detection task~\cite{mogelmose2014traffic}.  Such networks are often used in autonomous driving tasks, where a misclassification of a traffic sign could prove fatal.
% The poison patterns used include a picture of a bomb, of a flower, and a simple yellow square.
% By using non gradient-perturbation based patterns, the defender can no longer rely on techniques based on detecting adversarial perturbational patterns (several of which are listed in Section \ref{sec:related_work}).
% Furthermore, this attack has been shown to be effective even when the model is retrained in a transfer-learning setting, meaning vulnerabilities can propogate through multiple networks and are not necessarily mitigated by model retraining. 
% Deep learning practioners often utilize pre-trained models to fine-tune on particular tasks~\cite{papernot2016semi}, meaning such an attack could be practically deployed with current model-sharing practices.\GP{This is a very detailed presentation. Not sure if we need to detail the specific algorithm used. Here, we need to make sure that the reader understands the "what" the attacker could do by modifying weights, not the "how".}

% \subsubsection{Model Modification Attacks}
% A model without access to the training data or phase can still modify the network to respond to specified adversarial attacks.  This opens up problematic concerns as a deployed model in an unsecured environment can be intercepted by the attacker before re-deployment.  Though some works explore the usage of verification techniques for neural networks~\cite{he2018verideep} to ensure a model has not been tampered with, these techniques have not been widely adopted by the community and prohibits the practitioner from updating or tweaking the model after verification.

% The algorithm in Trojaning Neural Networks~\cite{Liu2018TrojaningAO} selects a few neurons in a neural network to generate a patch of adversarial perturbations, called a 'trigger'. 
% This is distinct from most adversarial perturbation work, where an output is targeted to obtain the gradient noise.  
% The last few layers of the model are then retrained with synthetic data to respond to the trigger to activate a certain output, a process which is considerably faster than training an entire network from scratch and which does not require the use of the original training data.
% The procedure also does not significantly change the behavior or affect the performance of the model.
% An already-deployed model can thus be tampered with and redeployed, ready to respond to a trigger known only to the attacker.  
% There are some unique design challenges that arise for the defender. 
% Some defenses generate anticipated adversarial attacks to train a classifier network to detect adversarial inputs (see Section \ref{sec:related_work}), but because the attacker only chooses specific secret neurons for trigger generated, the defender will not be able to generate data needed to train the classifier. 
% Third party classifier or detector networks will also be thwarted, as the trigger is designed to only affect the target model.   
% The attack is deployed in various settings, include facial recognition, speech recognition, and sentiment classification tasks.\GP{Same as before, focus on the "what", not on the "how".}

% \subsubsection{White-box/Black-box attacks}
% Works have shown that an attacker can successfully fool a model without access to the training phase or modifying the model.  This means that under the most secure conditions where the model's provider and training data can be trusted, our model is still vulnerable to localized adversarial attacks due to the inherent properties of convolutional neural networks. 

% Adversarial Patches~\cite{brown2017adversarialpatch} use adversarial perturbations targeted towards a specified output and limited to a small region of the image.  
% The attack was demonstrated on Imagenet~\cite{deng09imagenet} trained networks.
% The generated patches are designed to be robust, able to cause misclassification of arbitrary images and to work in real-world conditions with different lighting or angles.  A compelling capability of the adversarial patch is its ability to cause misclassifications across multiple Imagenet models with very different architectures.
% The paper demonstrates that even if the attacker lacks white-box access to the model, an attack can be generated using different models trained to perform the same task. 
% Therefore, an attack is possible even in a setting where the model's source can be trusted through use of integrity-protection techniques like Verideep~\cite{he2018verideep}, and even if the attacker doesn't have access to the model or knowledge of its architecture.\GP{This one is good.}

% \subsection{Overview} The attacks above all vary in attack mechanism and thus effect the model different, making detection difficult.  Furthermore, the attacks listed above can all use adversarial shapes that can vary greatly in size, shape, and placement.  With all this in mind, we now have a picture of what a good defense should entail.  Under this threat model, security should be ensured without knowledge of an attack's appearance, mechanism, or the condition of the target model. \GP{I think we need to say something more about the properties of the malicious input we are looking for. We may want to have a subsection that defines precisely the notion of localized malicious input.}


 

==> Archive 2/conclusion.tex <==
% !TeX root = ./main.tex
\section{Conclusion}
\label{sec:conclusion}

In this work, we introduce \tool{}, a framework for detecting localized universal attacks on Convolutional Neural Networks.  Our method is notable because it only relies on the malicious behavior of an adversarial attack to perform classifications, without requiring prior knowledge of the attack vector.  We demonstrate the versatility of \tool{} on three experiments with fundamentally different attack mechanisms: a data poisoning attack, a network trojaning attack, and adversarial patches---including physically realizable ones.  We further evaluate the robustness of \tool{} against strong adaptive adversaries by individually testing each component of our defense.  Our approach can be run in realtime in many scenarios, and is flexible and easy to deploy.

% There are further improvements that would help improve the performance of \tool{}.  Better visualization techniques (see, e.g., Grad-CAM++~\cite{chattopadhyay2017gradcamplus}) would improve the heatmap quality to create better masks. Deep learning interpretability and visualization is a challenging problem and breakthroughs in this area can also allow us to further reason about whether an attack is taking place.  Furthermore, our anomaly detection approach can be further extended to take advantage of the richer data provided by the neuron outputs during the inference process.  Works have shown techniques to detect anomalous high dimensional data using one class neural networks (see, e.g.,~\cite{goldstein2016anomaly,chalapathy2018anomalyoneclass}) which could enhance our current framework.

We hope \tool{} inspires further approaches towards creating attack-agnostic defenses.  Tailoring a defense towards a specific attack means unknown attacks cannot be captured, and also makes the system highly vulnerable to strong adaptive adversaries. We believe a similar approach can be used to detect other attacks by leveraging the same core concepts of identifying an attack from a model's weakness.


==> Archive 2/discussion.tex <==
% !TeX root = ./main.tex
\section{Discussion}
\label{sec:discussion}

Our results show that our defense is able to record high accuracy metrics for detecting adversarial images in all three cases and is robust to strong adaptive adversaries.  We now discuss in more depth the strengths and limitations of our approach, highlighting some unusual aspects of our design.

%\subsection{Strengths of our Defense}

\paragraph{Attack Detection} We showed the effectiveness of \tool{} when protecting both compromised and uncompromised networks, without prior knowledge of the network vulnerability. Attack detection rates in four attacks are between 98.5\% and 99.2\%. In one attack, \tool{} scored 85.5\% TP rate, that is comparable with proposed detection techniques~\cite{carlini2018eval}.

\paragraph{Turning a Weakness into a Strength and Proportional Defense} One strength of \tool{} is that it relies on the fact models are compromised by an attack.  Therefore, our detection framework is largely unaffected by the mechanism or deployment the attack uses, detecting attacks successfully as long as they fool the model.  In fact, \tool{} is better at detecting attacks when the adversary is stronger. The properties that characterize a strong attack make it easier for \tool{} detection as such an attack would easily result in outlier behavior outside the threshold of an approximated curve. In real-world conditions, attacks have to be even more robust as they need to tolerate different lighting and viewpoint variations.  Real-world deployments of neural networks could potentially represent the most potent deployment scenario for \tool{}.

\paragraph{Detection of Unsuccessful Attacks} \tool{} can also be further extended with additional functionality.  With the adversarial input detection and class proposal, \tool{} can also analyze the second or subsequent proposed classes, raising the possibility of using \tool{} to detect unsuccessful, attempted attacks. Such a behavior can be useful and help deter attackers from probing and testing our defense with experimental attacks.

\paragraph{Runtime Adversarial Object Suppression} Furthermore, the masking functionality can be used to still preserve functionality by reporting the output label with the inert pattern.  Unlike other detection frameworks which simply identify when an attack has taken place, the calculated mask of \tool{} can easily be used to remove the localized universal attack and salvage as much of the rest of the data as possible. 

%\subsection{Limitations of our Defense}\label{sec:limitations}

% \spreview{Adversarial problem is hard - lots of defense have been proposed
% Shouldn’t expect a simple and easy solution
% Focus on a simple and realistic threat
% Insist on this, make it very clear.
% Think about this a bit more, make this stronger
% }

% \paragraph{Small Adversarial Objects}---One flaw of \tool{} is its reliance of the correctness of the Grad-CAM visualization behavior.  We have observed a decrease in \tool{} performance when the when the Grad-CAM heatmap granularity is insufficient. Smaller attacks will likely cause issues with Grad-CAM as with the coarse heatmap capturing too much information around the actual attack pixels.\GP{Too negative, we are giving ammos to reviewers. Give a more positive spin.}

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{sentinet_figs/imagenet_size_400_none.png}
	\caption{Size analysis of adversarial patches. The legend denotes the ratio of the image to the input, and we can see that the $AvgConf$ drops as the size increases.  On the right, we plot the attack success rate after increasing the transparency values, and we can see that with large ($> 0.35$) patches the input drops below the decision boundary while still retaining a 90\% attack success rate.}
	\label{fig:size_analysis}
\end{figure}

\paragraph{Attack Size} The goal of \tool{} is to capture unreasonably salient attacks, designed to be small and unnoticeable. With this measure, \tool{} largely succeeds at detecting abnormal regions of images that deviate from patches of natural images. When adversaries can modify the majority of pixels in an image, they can override the prediction. As noted by Brown et al.~\cite{brown2017adversarialpatch}, large images of an actual toaster will hijack the same prediction of an adversarial patch at a large enough size, raising an interesting question about what actually constitutes an ``attack''. Based on this observation, we note that the attack's $avgConf$ drops as the size of the object increases, and by increasing the transparency of the object, the attack drops below the threshold while retaining very high attack success (See \Cref{fig:size_analysis}). Similarly as observed by Brown et al.~\cite{brown2017adversarialpatch}, drop of $avgConf$ and high attack success is the result of obfuscating the test inputs with the large targeted class. We conclude that, while our defense correctly captures small patches, the detection of unreasonably large objects is very challenging for \tool{}. 

% In general, adversaries can override an image prediction if they are allowed to modify the majority of pixels in an image. \tool{} makes the assumption that adversarial objects are small. We show in Section \ref{sec:evaluation} that large enough patches can easily bypass the decision boundary of our model.  However, we note once more that Brown et al.~\cite{brown2017adversarialpatch} demonstrates how large images of toasters will hijack the prediction of classification models, which is expected behavior even for a human classifier.  In general, if an attacker can modify a majority of an image, it is trivial to influence the output by obfuscating the input with the targeted class. Our focus with \tool{} is to capture adversarial attacks that are unreasonably salient, designed to be small and unnoticeable and that would not fool humans. With this measure, \tool{} largely succeeds at detecting abnormal regions of images that deviate from patches of natural images.
% \GP{Too negative (we talk about flaw), give a more positive spin (perhaps talk about the property with large adversarial objects which is an obvious behavior when the majority of pixels is adversarial)}

% If an attack manages to avoid being detected in the heatmap altogether, it can bypass \tool{} completely. However, our mask reduction approach at least mitigates the likelihood of too-large heatmaps, and an attacker would have to find a way to cause their adverarial region to not be highlighted by Grad-CAM altogether. 

% \paragraph{Non-Targeted Attacks}---Another potential flaw of the current \tool{} approach is assumptions that are made about the attack behavior.  In the adversarial patch and trojaning network attack, the adversarial attacks will cause misclassifications towards one particular class, while BadNets will always cause a misclassification of one class to another class.  There are other possible behaviors that the attacker could be attempting to produce.  Two especially problematic scenarios would be attacks that simply cause an erroneous misclassification rather than a misclassification towards a specific class, and an attack that is only designed for one particular image and does not generalize to other images even within the same class.  For the first case, we can see how our current \tool{} setup can be adjusted to set $numFooled$ as the number of misclassifications overall rather than the number of targeted misclassifications, but it is likely that the attack will be less effective overall as many non-adversarial patches could cause misclassifications when overlaid onto other images.  Similarly, in the second case, we can adjust the the approach to measure the differences of network behavior with the localized adversarial overlay, but there is a similar issue where confidently predicting an attack would be difficult.  We can see that issue slightly in BadNets, where the accuracy metrics are lower due to the attack only causing misclassifications of one label rather than of images with arbitrary labels.\GP{We should drop this and clarify that non-targeted attacks (random errors) are not part of our threat model}

% \paragraph{Weak Attacks}---
% One interesting aspect of \tool{} is its potential ability to create a new type of localized adversarial attack.  The FP adversarial attacks found by \tool{} fool many test images and do not obfuscate important regions of other images.  If one uses these False Positive examples found as a localized adversarial patch, the user has created an attack that is natural while having similar properties as a synthetically generate attack.  In effect, this approach discovers the biases ingrained in the model and utilizes objects within a training or test set to fool the model.  \tool{} will struggle to accurately classify such attacks, as their behaviors will more likely be within normal bounds of clean examples.  With models and datasets that are especially biased, the variance in behavior of the clean samples will likely significantly overlap with an actual attack. Indeed, the other attacks can also be modified reduce the effectiveness in order to escape \tool{} detection.  Adversarial patches or trojaning triggers designed to cause less misclassifications or to take up larger sizes can bypass a \tool{}-type approach.  Having an defense mechanism that forces the attacker to reduce the power of the attack is still of value however.  Literature introducing new localized adversarial attacks tend to frame the ability to cause misclassifications reliably and to not be able to placed surreptitiously in the background as strengths of their approach, and \tool{} could potentially cap how effective an attack can be.\GP{Not sure I understood the point. Needs a second pass.}

% \paragraph{Patterns Targeting Different Classes}---When an attacker places multiple patches into the image targeting different classes, our defense will capture one of the patches, leaving the other patch to pass through undetected. To fix this behavior, \tool{} could run iterations of our defense until the image is no longer classified as an adversarial by adding a linear increase in runtime for each additional patch.

%%%%
%% 1) Our meas. w/ optimistic estim. of class proposal w/ Titan X:
%%    (a) selective search + class proposal = 2.34s
%%    (b) selective search                  = 2.3s
%% 2) From YOLO + Github
%%    (c) selective search + class proposal = 2s
%%    (d) selective search                  = (c)*(a)/(b) = 1.97s
%%  
%% Estimated ratio selective search / total = (d)/(c) = 99%
%%%%

\paragraph{Latency} The runtime of \tool{} is about 2.5s, which is acceptable for tasks like runtime facial recognition. However, it could be impractical for real-time scenarios including autonomous driving. The vast majority of the runtime of \tool{} (1.9s, i.e., ~75\% of the total) is taken by the selective search algorithm. Over the past years, the research community has proposed faster image segmentation approaches; however, none of the new ideas seem to offer the same trade-off between precision, performance, and security as provided by the selective search algorithm. For example, Ren et al.~\cite{ren2015fasterrcnn} and Redmon et al.~\cite{redmon2015yolo, redmon2016yolo9000, redmon2018yolov3} proposes using a neural network to segment images. These new approaches are remarkably fast, taking as little as 0.02 seconds per image (i.e., YOLOv3~\cite{redmon2018yolov3}) to segment an image. While such a low runtime is very desirable for \tool{}, neural network segmentation algorithms introduce severe vulnerabilities in \tool{}. For example, in a recent work, Tram\`{e}r et al.~\cite{tramer2018ad} showed an interesting property of neural network image segmentation techniques, where an adversary can use perturbations to fully control the position and the size of the output segments. Alternatively, in scenarios where efficiency is a priority, a sliding-window approach can be a valid alternative. However, the sliding-window approach has a few drawbacks that make it inadequate for \tool{}. Specifically, it improves execution time only when using large windows, and large windows are more likely to contain multiple classes, affecting the capability to detect adversarial inputs of \tool{}. Overall, based on the current state of the art, we believe selective search is adequate to cope with relevant deployment scenarios of DL systems. Also, we hope that the encouraging results of \tool{} will inspire researchers to propose more efficient and secure segmentation techniques.

\paragraph{Other Classes of Attacks and Future Improvement} The goal of \tool{} is to protect networks against localized universal adversarial inputs, and our results show the viability and robustness of our approach. However, other types of attacks may be possible such as non-universal malicious objects, e.g., patches that work with specific images, or non-localized malicious objects, e.g., disjoint patches. These attacks may pose a challenge for \tool{} and their impact needs to be further studied. 

A promising direction that could improve \tool{} to handle disjoint malicious objects is using other finer-grained visualization techniques, e.g., Grad-CAM++~\cite{chattopadhyay2017gradcamplus}. In general, deep learning interpretability and visualization is a challenging problem and breakthroughs in this area can also allow us to further reason about whether such attacks will take place. 

Handling non-universal patches may require to revisit the anomaly detection phase, which assumes that successful attacks hijack test inputs of different classes. The anomaly detection approach of \tool{} could be extended to take advantage of the richer data provided by the neuron outputs during the inference process. Recent works have shown techniques to detect anomalous high dimensional data using one class neural networks (see, e.g.,~\cite{goldstein2016anomaly,chalapathy2018anomalyoneclass}) which could enhance our current framework.

% \paragraph{Overhead}---The runtime of our approach is 7.7s, ${\sim}$3x a forward pass of the original network. While the current runtime of \tool{} is acceptable for tasks like run-time facial recognition, it could be impractical for real-time scenarios including autonomous driving. However, we note that the measured runtime is largely overapproximated, and it has to be seen as an upperbound value for the following two reasons. First, our experiments' runtime of a single evaluation of a network is very high when compared to the tens of milliseconds with optimized hardware and software configurations. Accordingly, we can expect that ad-hoc configurations can push the two forward pass performed by \tool{} below a second (i.e., Forward Pass and Class Proposal of \Cref{tab:runtime_analysis}). Second, selective search is run on CPU and it counts for a third of the total measured runtime, rendering it the slowest component of \tool{}. Porting selective search on GPU could improve the runtime, however, the nature of the algorithms used by selective search may not fully benefits from it. 

%\paragraph{Overhead}---The runtime of our approach is 7.6s, ${\sim}$3x the original computation time.  Each inference requires a constant overhead, raising the inference time from milliseconds to several seconds.  This lag for real-time detection scenarios is perhaps acceptable for tasks like facial recognition, but could prove impractical in scenarios including autonomous driving.  However, the computational cost is more relevant, as instead of performing one forward pass through our network, \tool{} performs hundreds of batched inferences.  In non real-time situations, it is common for inference to be performed in batches, that in our case a batch has 100 images.  This would be incompatible with the current \tool{} setup, as for each input \tool{} will require 100 additional inputs during each fuzzing phase.  Performing parallel analysis is possible, requiring a proportional amount of memory a regular inference scheme is current using.  It is worth noting that many other detection schemes introduce significant overhead as well, and a small benefit of the \tool{} approach is its plug and play compatibility, only requiring a pre-computed run of small subset of clean samples.

==> Archive 2/evaluation.tex <==
% !TeX root = ./main.tex
\section{Evaluation}\label{sec:evaluation}

% \GP{what about an eval on the size of the patch/attack wrt of the input size?}

In this section, we evaluate \tool{} on a variety of previously proposed attacks, to highlight its versatility. In Section~\ref{sec:adaptive_attacks}, we then perform an extensive evaluation against \emph{adaptive} adversaries with full knowledge of \tool{}'s inner workings---thereby demonstrating \tool{}'s robustness.

After presenting the experiment setup in \Cref{sec:parameters}, in \Cref{sec:known_attacks}, we evaluate the effectiveness of \tool{} in protecting networks from three known attacks, i.e., adversarial patches, trojan triggers, and backdoors, with an average true positive rate of 96.22\% and an average true negative rate of 95.36\%. We further evaluate \tool{} in a realistic physical setting with a printed adversarial patch (see Section~\ref{sec:physical}).

Finally, in \Cref{sec:performance}, we look into the latency of \tool{} in terms of runtime analysis.

% \tool{} does not modify the original network through retraining or layer modification, and thus will not impact the performance of the network. Instead, it acts as a protection layer that determines whether the resulting output of the original network can be trusted. \tool{} needs to protect a network from adversarial inputs exploiting both inherent vulnerabilities of neural networks and implanted ones. \tool{} is executed after the model prediction involving operations including the Grad-CAM visualizations, the selective search algorithm, and multiple evaluations of the network under protection. As a result, as \tool{} adds overhead between the classification and the actuator, \tool{} needs to be efficient.

% In this section, we evaluate \tool{} covering these two dimensions. After presenting the experiment setup in \Cref{sec:parameters}, in \Cref{sec:known_attacks}, we evaluate the effectiveness of \tool{} in detecting three known attacks, i.e., adversarial patches, trojan triggers, and backdoors. Finally, in \Cref{sec:performance}, we look into the performance overhead of \tool{} in terms of wallclock and runtime analysis.

\subsection{General Experiment Settings}
\label{sec:parameters}


We evaluated \tool{} when protecting three publicly available networks shared from prior works. Two of the selected networks are compromised and one is uncompromised. The compromised networks are a backdoored Faster-RCNN network for reading signs detection by Gu et al.~\cite{gu2017badnets} and a VGG-16 trojaned network for facial recognition by Liu et al.~\cite{Liu2018TrojaningAO}. The uncompromised network is a VGG-16 network trained on the Imagenet dataset by Simonyan et al.~\cite{simonyan2018vgg16}. Additionally, to operate, \tool{} requires a benign test image set $X$ and an inert pattern $s$ to generate the decision boundary as shown in \Cref{sec:fuzzing}. We present the generation of each test set $X$ for the selected networks in \Cref{sec:known_attacks}. Unless specified, we use random noise for our inert pattern $s$.

We measure the effectiveness and robustness of \tool{} in terms of accuracy and performance, collecting the TP/TN and FP/FN rates of \tool{} when processing benign and adversarial inputs. We present the creation of benign and adversarial images datasets of our experiments in \Cref{sec:known_attacks}. We measure efficiency by evaluating the execution of each step of \tool{}.

Finally, %we evaluated \tool{} using a Tesla K-80 GPU on an Ubuntu 18.04 machine with Intel Xeon CPU E5-2697 and 72 cores. 
\tool{} uses Tensorflow 1.5 to generate the adversarial patches for the uncompromised network, BLVC-Caffe for the trojaned network, and Faster-RCNN Caffe~\cite{girshick2015fastrcnn} for the poisoned network. To parallelize the class proposal, \tool{} relies on the ROI pooling layer as implemented by the Fast-RCNN Caffe version. Finally, \tool{} uses the off-the-shelf implementations of Grad-CAM~\cite{selvaraju2016gradcam} and selective search~\cite{uijlings2013selectivesearch}.



\subsection{Effectiveness}
\label{sec:known_attacks}

The first part of our evaluation assesses the effectiveness of \tool{} in protecting our selected networks against three attacks, i.e., trojan triggers~\cite{Liu2018TrojaningAO} against trojaned networks, backdoors~\cite{gu2017badnets} against poisoned networks, and adversarial patches~\cite{brown2017adversarialpatch} against uncompromised models. For each attack, we measured the effectiveness of \tool{} in terms of the number of attacks detected. For the adversarial patches attack, we considered an additional variant where the attacker uses multiple patches at the same time. The summary of this evaluation is in \Cref{tab:known_attacks_results}.

% \begin{table*}
%     \centering
% 	\begin{tabular}{l l l c c c c c }
%         \toprule
%         \textbf{Network}      & \textbf{Vuln.} & \textbf{Attack} & \textbf{Source}                    & \textbf{TP} & \textbf{TN} & \textbf{FP} & \textbf{FN} \\

%         \midrule
%         VGG-whatever & Trojaned & Attack \#1, w/o mask reduction & \cite{Liu2018TrojaningAO} & 100\% & 100\% & 0\% & 0\%\\
%         VGG-whatever & Trojaned & Attack \#1  & \cite{Liu2018TrojaningAO} & 100\% & 100\% & 0\% & 0\%\\
%         CNN-whatever & Poisoned    & Attack \#2 & \cite{gu2017badnets} & 100\% & 100\% & 0\% & 0\%\\
%         What!?GG-whatever & Uncompr. & Attack \#3 & \cite{Liu2018TrojaningAO} & 100\% & 100\% & 0\% & 0\%\\
%         What!?GG-whatever & Uncompr. & Attack \#4 & \cite{Liu2018TrojaningAO} & 100\% & 100\% & 0\% & 0\%\\
%         \bottomrule
%     \end{tabular}
%     \label{tab:known_attacks_results}
%     \caption{Evaluation of \tool{} against three known attacks.\GP{I would collect all resuls in a table like that}}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                    RAW DATA
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Face square (random)
% True Positive: 0.991848 (detected: 365, total: 368)
% True Negative: 0.997500 (passed: 399, total: 400)
% 
% Face square (checker)
% True Positive: 0.991848 (detected: 365, total: 368)
% True Negative: 0.995000 (passed: 398, total: 400)
%
% Adversarial patch: 
% True Positive: 0.985207 (detected: 333, total: 338)
% True Negative: 0.952500 (passed: 381, total: 400)
%
% X2 adversarial patch: 
% True Positive: 0.997290 (detected: 368, total: 369)
% True Negative: 0.950000 (passed: 380, total: 400)
%
% Poisoned network: 
% True Positive: 0.850746 (detected: 114, total: 134)
% True Negative: 0.868966 (passed: 126, total: 145)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
	%\footnotesize
	\centering
	\caption{Effectiveness of \tool{} protecting compromised and uncompromised networks.}
	\begin{tabular}{l l l c r r r r}
		\toprule
		\textbf{Network and Task}                                 & \textbf{Attack}            & \textbf{Inert Noise} & \multicolumn{1}{c}{\textbf{TP}} & \multicolumn{1}{c}{\textbf{TN}} & \multicolumn{1}{c}{\textbf{FP}} & \multicolumn{1}{c}{\textbf{FN}} \\

		\midrule
		VGG-16~\cite{Liu2018TrojaningAO} for face recognition     & Trojan trigger             & Random               & 99.2\%                          & 99.8\%                          & 0.3\%                           & 0.8\%                           \\
		VGG-16~\cite{Liu2018TrojaningAO} for face recognition     & Trojan trigger             & Checker              & 99.2\%                          & 99.5\%                          & 0.5\%                           & 0.8\%                           \\
		Faster-RCNN~\cite{gu2017badnets} for road signs detection & Backdoor                   & Random               & 85.0\%                          & 86.9\%                          & 13.1\%                          & 14.8\%                          \\
		VGG-16~\cite{simonyan2018vgg16} for ImageNet              & Adversarial patch          & Random               & 98.5\%                          & 95.3\%                          & 4.8\%                           & 1.5\%                           \\
		VGG-16~\cite{simonyan2018vgg16} for ImageNet              & 2$\times$Adversarial patch & Random               & 99.2\%                          & 95.3\%                          & 4.8\%                           & 0.8\%                           \\
		VGG-16~\cite{simonyan2018vgg16} for ImageNet              & Physical adversarial patch & Random               & 93.7\%               & 90.2\%                & 9.8\%                & 6.3\%                \\
		\bottomrule
	\end{tabular}
	\label{tab:known_attacks_results}
\end{table*}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.35\columnwidth]{figures/flower_nobg.png}
% 	\includegraphics[width=0.35\columnwidth]{figures/badnets_qualitative.png}\\   \vspace{0.25cm}
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/traffic_poison_attack_usstop_test_all_145_origpred.png}
% 	\caption{The top row shows the backdoor, i.e,. a flower, and the Grad-CAM output for the class ``warning-sign'' on an adversarial stop sign. The bottom row shows the decision boundary generated of the poisoned network. The blue circles denote benign inputs and the red triangles denote adversarial inputs.}
% 	\label{fig:badnets_qualitative}
% \end{figure}


\subsubsection{Trojaned Networks}
%\vspace{0.1cm}\noindent\textbf{Attack \#2: Trojaned Networks}---

A trojaned network is a model whose weights have been modified by an adversary to implant a response when processing inputs containing a so-called \emph{trigger trojan}~\cite{Liu2018TrojaningAO}. The trigger trojan is created from a set of specified neurons, and then fine-tunes the model's weights on the trigger to hijack the prediction~\cite{Liu2018TrojaningAO}. For our evaluation, we selected the facial recognition model shared by Liu et al.~\cite{Liu2018TrojaningAO} with a VGG-16 architecture~\cite{simonyan2018vgg16} trained on the VGG-Face dataset~\cite{parkhi2015vggface}.

\paragraph{Datasets} For the evaluation, we created three datasets with benign, adversarial, and test images as follows. The benign images dataset contains 400 images randomly selected from the LFW dataset~\cite{huang2007lfw}. From the benign dataset, we derived the adversarial inputs dataset by placing the square trigger trojan shared by Liu et al.~\cite{Liu2018TrojaningAO} to hijack the prediction of the VGG-16 network to the class ``A.J. Buckley''. As the trigger trojan is created from a fixed region of the input, we placed them in the same position, i.e., the bottom-right corner of each image.  An example of such a trigger trojan and adversarial input is shown in \Cref{fig:trojan_qualitative}. Then, the test set $X$ contains 100 randomly selected images from the VGG-16 dataset~\cite{simonyan2018vgg16}. Finally, in this evaluation, we considered two types of inert noise, i.e., random noise and checker pattern (Examples of the two types of inert noise are in \Cref{fig:secret_patterns}).

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\columnwidth]{figures/random_noise.png}~
	\includegraphics[width=0.48\columnwidth]{figures/checker_pattern.jpeg} \\
	\caption{Examples of inert patterns. The default pattern we use for $s$ is random noise shown on the left.  Another pattern we can potentially use is the checkered pattern on the right which the VGG-Face network also responds weakly to.}
	\label{fig:secret_patterns}
\end{figure}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{.234\linewidth}
		\centering
		\includegraphics[width=0.48\columnwidth]{figures/trojan_cropped.png}
		\includegraphics[width=0.48\columnwidth]{figures/face_trojan_another.png}\\
		\vspace{0.45cm}
		\includegraphics[width=1\columnwidth]{sentinet_figs/face_square_400_origpred.png}
		\caption{Trojan trigger.}
		\label{fig:trojan_qualitative}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{.235\linewidth}
		\centering
		\includegraphics[width=0.48\columnwidth]{figures/flower_nobg.png}
		\includegraphics[width=0.43\columnwidth]{figures/badnets_qualitative.png}\\
		\vspace{0.45cm}
		\includegraphics[width=1\columnwidth]{sentinet_figs/traffic_poison_attack_usstop_test_all_145_origpred.png}
		\caption{Backdoor.}
		\label{fig:badnets_qualitative}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{.234\linewidth}
		\centering
		\includegraphics[width=0.48\columnwidth]{figures/adversarial_patch.png}
		\includegraphics[width=0.48\columnwidth]{figures/imagenet.png}\\
		\vspace{0.45cm}
		\includegraphics[width=1\columnwidth]{sentinet_figs/imagenet_400_origpred.png}
		\caption{Adversarial patch.}
		\label{fig:adversarialpatch_qualitative}
	\end{subfigure}\hfill
	\begin{subfigure}[b]{.234\linewidth}
		\centering
		\includegraphics[width=0.48\columnwidth]{figures/imagenet_double.png}
		\includegraphics[width=0.48\columnwidth]{figures/imagenet_double_859.png}\\
		\vspace{0.45cm}
		\includegraphics[width=1\columnwidth]{sentinet_figs/imagenet_double_400_origpred.png}
		\caption{2$\times$Adversarial patch.}
		\label{fig:double_qualitative}
	\end{subfigure}
	\caption{Evaluation inputs and results. The first row shows examples of adversarial objects used by the attacker and the Grad-CAM output. The bottom row shows scattered plots of benign inputs (in blue) and adversarial inputs (in red) with respect to the decision boundaries (solid lines) and thresholds (dashed lines) used by \tool{} for the attack detection.}
	\label{fig:evaluation_results}
\end{figure*}

% A trojaning attack generates a trigger from specified neurons in the network, and then fine-tunes the model on the trigger to respond to a specific output. The generated trigger can be created with any shape or size using both convolutional and fully-connected neurons.  The trojaned model for our target network $f_m$ is the facial recognition model shared by Liu et al.~\cite{Liu2018TrojaningAO} with a VGG-16 architecture~\cite{simonyan2018vgg16} trained on the VGG-Face dataset~\cite{parkhi2015vggface}. In the evaluation, we used the square trigger that can be generated with neurons from the FC6 layer of the VGG-16 network. This trigger hijack the prediction of the VGG-16 network to class 0, i.e., ``A.J. Buckley''. We use a separate facial recognition dataset to generate our clean and adversarial datasets. We use 400 examples of the LFW dataset~\cite{huang2007lfw}, placing the trigger of each of these images. Of the 400 adversarial images,
% 368 of them successfully direct the output of the model to class 0. Our test set $X$ consists of 100 images from the original VGG-16 dataset~\cite{simonyan2018vgg16}.

\paragraph{Results} Of the 400 adversarial images, 368 of them hijack the prediction of the compromised model, i.e., the model incorrectly predicted ``A.J. Buckley''. Of these 368 attacks, \tool{} can successfully detect almost all of them. i.e., 365 malicious inputs resulting in TP rates above 99\%, regardless of the used inert noise. Then, the number of TN is also considerably high, with rates above 99\%. In this case, the inert noise has a very marginal role in the detection. Of the 400 benign images, we have one FN when using the random inert noise and two FNs when using the checker inert noise.

To better understand the behavior of \tool{}, we have a closer look at the distribution of the benign and adversarial images with respect to the decision boundary used by \tool{}. The plot is shown in \Cref{fig:trojan_qualitative}. As expected, most of the benign samples (in blue) fail to fool the model except for few outliers which produce low $avgConf$ scores. On the contrary, the adversarial inputs (in red) fool the model a high number of times with a very high $avgConf$ confidence scores. The decision boundary is calculated using the test set $X$ as explained in \Cref{sec:fuzzing}, and it is well separating the adversarial from benign regions.

% We note that CanaryNet is particular effective for this specific attack.  This is likely due to the nature of both the dataset and the trigger placement; a face recognition dataset consists of many images with faces with roughly the same size and orientation, while this particular trigger aims to cause misclassification without covering the main parts of a face.  As long as CanaryNet successfully isolates the attack region, the $numFooled$ and $avgConf$ metrics will likely be greatly different due to the nature of the dataset.

%GP: Commented out
%In this task, we can also see the greater importance of our mask reduction technique.  The trojan mechanism in particular seems work with the combination of both trigger and the original facial regions. This often results in the Grad-CAM highlighting regions outside the trigger. \Cref{tab:known_attacks_results}, we can see the clear improvement Mask Reduction has on improving the True Positive and True Negative rates of \tool{}.\GP{Drop mask reduction?}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.40\columnwidth]{figures/adversarial_patch.png}
% 	\includegraphics[width=0.40\columnwidth]{figures/imagenet.png}\\   \vspace{0.25cm}
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/imagenet_400_origpred.png}
% 	\caption{The top row shows the adversarial patch by Brown et al.~\cite{brown2017adversarialpatch} and the Grad-CAM output of ``toaster'' on a randomly chosen adversarial image. The bottom row shows the decision boundary. The blue circles denote benign inputs and the red triangles denote adversarial inputs.}
% 	\label{fig:adversarialpatch_qualitative}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/imagenet_400_origpred.png}
% 	\caption{object detector}
% 	\label{fig:adversarialpatch_decisionboundary}
% \end{figure}

%\vspace{0.1cm}\noindent\textbf{Attack \#3: Adversarial Patches}---

%\vspace{0.1cm}\noindent\textbf{Poisoned Networks}---

\subsubsection{Poisoned Networks}

A poisoned network is a model created by an adversary via training, with the goal to implant a specific model response when processing inputs containing a \emph{backdoor}. As opposed to trojaned networks, poisoned networks are compromised \emph{during} the training phase instead of after. For our evaluation, we selected the poisoned network shared by Gu et al.~\cite{gu2017badnets}, a Faster-RCNN model~\cite{ren2015fasterrcnn} to detect stop signs. The authors poisoned the training set so that the network will incorrectly classify stop signs with a yellow flower---the backdoor---as a warning sign. The backdoor and an example of adversarial input is shown in \Cref{fig:badnets_qualitative}.

\paragraph{Datasets} For this evaluation, the benign images dataset contains 145 images of stop signs from the LISA dataset~\cite{mogelmose2014traffic} by cropping out the images with their labeled bounding boxes. Then, we derived the adversarial images by placing the yellow flower backdoor shared by Gu et al.~\cite{gu2017badnets} at approximately below the ``stop'' text of each sign to create an ``attack'' dataset. The test set $X$ contains 100 images selected from each class with equal probability.

% For our evaluation, we create the boundary decision as described in \Cref{sec:fuzzing}. 

\paragraph{Results} Out of the 145 adversarial inputs, 134 images successfully fool the Faster-RCNN model. \tool{} detected 114 images, with a TP rate of 85\%. When using benign images, \tool{} incorrectly detected 19 images of 145 benign inputs, resulting in a 14.8\% FNs. While \tool{} can achieve much higher accuracy and precision, we note that \tool{}'s accuracy in this experiment is comparable to the accuracy of proposed adversarial detection techniques (see, e.g.,~\cite{carlini2018eval}).

Higher FP and FN rates of \tool{} can be better explained by having a look at the distribution of benign and adversarial images in \Cref{fig:badnets_qualitative}. As opposed to trojaned networks, benign and adversarial images are not densely grouped. Instead, they are rather scattered over large areas, crossing the decision boundary in two points, i.e., benign images above the boundary decision in the center of the plot and adversarial inputs below the boundary decision. Scattered points as shown in \Cref{fig:badnets_qualitative} are likely due to coarser heatmaps generated by Grad-CAM when applied to the Faster-RCNN network. The Faster-RCNN architecture uses a 12 $\times$ 12 ROI pooling layer, whose layer is used by Grad-CAM to create the heatmap. The ROI pooling layer of the Faster-RCNN is smaller than the other networks used in our evaluation. For example, the VGG-16 trojaned network has a 16$\times$16 ROI pooling layer. A smaller ROI pooling layer results in coarser grained heatmaps, whose masks are likely to include regions unrelated to the targeted class. As a result, test images with overlaid adversarial regions will include ambiguous features affecting both the probability of fooling the network and the confidence of the classification.

% A significance aspect of this experiment is that the attack is non-perturbational, but rather a "natural" image of a flower.  Thus, unlike previous adversarial detection work, which often rely on detecting the "unnaturalness" of adversarial images or the different behaviors models exhibit with gradient perturbations, our technique will detect localized adversarial attacks regardless of how they are generated.  This is a more flexible approach towards detecting adversarial attacks, as our technique will theoretically work with attacks that do not yet exist and might not rely on perturbational noise.

% For our traffic detection task, because there are only three classes, we do not utilize the selective search approach to obtain the highest class candidates in order to reduce computational overhead; however, because the network already has a ROI pooling layer, such an implementation would not be challenging to implement. The BadNets implementation has additional overhead compared to the other cases due to the pyramid projection needed to produce the feature map. Because the inputs to the network have high variations in size, we cannot perform a batched mask operation, and instead of have to apply a resized mask to each image, a process we can accelerate with multithreading. Furthermore, we find that though the Faster-RCNN framework appears to support batched computations, batched inference in practice seem to produce inaccurate results, and also requires impractical amounts of compute for batches the size of 100.  It is worth noting that Faster-RCNN inputs are usually far larger than standard inputs for classification tasks, contributing to the overhead.  For our experiments, we perform the model fuzzing step in a sequential fashion.  The amount of overhead introduced by CanaryNets for the BadNets class is x seconds.

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.40\columnwidth]{figures/trojan_cropped.png}
% 	\includegraphics[width=0.40\columnwidth]{figures/face_trojan_another.png}
% 	\\
% 	\vspace{0.25cm}
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/face_square_400_origpred.png}
% 	\caption{The top row shows the trigger used by Liu et al.~\cite{Liu2018TrojaningAO} and the Grad-CAM output of ``A.J. Buckley'' on an a face of the actress Mary Astor with the trigger. The bottom row shows  the decision boundary. We use blue circles for benign inputs and red triangles denoting adversarial inputs.}
% 	\label{fig:trojan_qualitative}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/face_square_400_origpred.png}
% 	\caption{object detector}
% 	\label{fig:trojan_decisionboundary}
% \end{figure}

\subsubsection{Uncompromised Networks}
\label{sec:uncompr_networks_eval}

In this section, we evaluate \tool{} protecting an uncompromised network when processing adversarial patches. In our case, we use a VGG-16~\cite{simonyan2018vgg16} Imagenet-pretrained~\cite{deng09imagenet} network as our target network $f_m$.

\paragraph{Datasets} We randomly sampled 400 images from the Imagenet test set~\cite{deng09imagenet} to implement our attack. Then, we placed the patch at random positions on the 400 images to generate our dataset of adversarial images, occupying around 25\% of the input images. We used the adversarial patch created by Brown et al.~\cite{brown2017adversarialpatch} which can fool the Imagenet-trained VGG-16 model to classify inputs as a ``toaster''. The patch and an example of adversarial input is shown in \Cref{fig:adversarialpatch_qualitative}. Also, in this evaluation, we considered a variant of the attack with images containing multiple adversarial patches. Finally, our test set $X$ consists of 100 randomly selected images from the Imagenet training set.

\paragraph{Results} Our evaluation showed that 338 images of the 400 adversarial images with a single patch fool the Imagenet-trained VGG-16. \tool{} detected almost all of them, i.e., 333 out of 338 with a TP rate above 98\%. When using two patches, the adversary has a slightly higher advantage and can hijack the prediction 369 times over 400 attempts. Of these 369 attacks, \tool{} has a stronger response than single-patch attacks, detecting 368 attacks, with almost 100\% TP rate.

In \Cref{fig:adversarialpatch_qualitative,fig:double_qualitative}, we observe that the adversarial images (in red) points are skewed towards producing both higher $numFooled$ and $avgConf$ numbers. The classification rule generated by the decision boundary produces TN rates of ${\sim}$95\% as seen in \Cref{tab:known_attacks_results}. Overall, both TP and FP compare favorably to other literature focused on adversarial attack detection.

Finally, when using two patches simultaneously, Grad-CAM correctly identifies the two disjoint regions that contribute to the prediction. \Cref{fig:double_qualitative} shows both the heatmap and the mask generated by \tool{}. Additionally, we measured how often \tool{} can detect both patches by checking whether the generated masks are disjoint and cover substantial portions of both patches. We find that \tool{} discovers both patches 97.4\% of the time, which we consider to be sufficiently accurate relative to the TP and TN values.

\subsection{Physical Attacks}
\label{sec:physical}

Localized adversarial attacks have the distinct advantage of being deployable in real-world settings as a physical attack via stickers or patches, as compared to adversarial noise.  Several prior works~\cite{brown2017adversarialpatch, sharif2016glasses, evtimov2017robust, eykholt2018physical, athalye2017synthesizing} have demonstrated how adversarial noise can be effectively synthesized in the physical world to fool visual classifiers fed with video streams.
In this section, we experimentally validate that \tool{}'s defensive capabilities perform well in a realistic attack scenario where a physically printed patch is displayed next to a common object, with the goal of robustly and reliably subverting a classifier's predictions.

We captured a video of a banana displayed on its own or next to an adversarial patch~\cite{brown2017adversarialpatch} with a variety of positions and orientations (see Figure~\ref{fig:physical_atta}). The undefended VGG16 network classifies all $610$ benign video frames correctly, and is always fooled by the patch when present in all other $541$ frames. 
We evaluate \tool{} on these video frames using the same parameters as in our previous (digital) adversarial patch experiments---including the use of the randomly selected Imagenet test set and the checkerboard pattern for fuzzing. 
With \tool{}, the patch is correctly identified in $93.7\%$ of the video frames, and the banana is correctly identified in $90.2\%$ of benign frames.

Albeit not perfect, these results are promising: with \tool{}, the adversarial patch fails its goal of reliably subverting the classifiers on the vast majority of frames. In a deployment scenario where a classifier averages predictions over multiple frames (e.g., by yielding an object prediction every $10$ frames, via a majority vote over the preceding frames), \tool{} successfully yields correct classifications for the full benign video, while detecting and rejecting the adversarially perturbed video.

% The higher variance of values for the clean dataset (blue points) could be characteristic of the Imagenet dataset and task, where it is likely that some natural objects will cause abnormally numbers of misclassifications when segmented out and placed onto other images. 

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.40\columnwidth]{figures/imagenet_double.png}
% 	\includegraphics[width=0.40\columnwidth]{figures/imagenet_double_859.png}\\   \vspace{0.25cm}
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/imagenet_double_400_origpred.png}
% 	\caption{The top row shows the Grad-CAM output of ``toaster'' with disjoint adversarial patches and the generated mask.  The bottom row shows the decision boundary. The blue circles denote benign inputs and the red triangles denote adversarial inputs.}
% 	\label{fig:double_qualitative}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/imagenet_double_400_origpred.png}
% 	\caption{object detector}
% 	\label{fig:double_decisionboundary}
% \end{figure}



% \vspace{0.1cm}\noindent\textbf{Attack \#4: Multiple Adversarial Patches}---As an extension of Attack \#3, we perform experiments on images containing multiple adversarial patches, using the same target network $f_m$ and patch from Attack \#3. The setup is largely the same as the previous setting, except that two slightly smaller patches are randomly placed on opposing sides of an image.  This experiment is mainly performed to highlight \tool{}'s generalizability to detect attacks that are unpredictable in deployment and appearance.  Being able to detect disjoint attacks is a great demonstration of the ability of our model to identify attacks without any prior knowledge of the adversary.

% Grad-CAM can be used to visualize disjoint regions of an image that contribute towards the same class. As we can see in \Cref{fig:double_qualitative}, this applies to adversarial patches, with both patches successfully highlighted in the attack example. We do not have to modify our technique to make \tool{} work in this scenario.  We use a random sample of 400 images from Imagenet test set to create our dataset (we also use 100 images from Imagenet train set as test set $X$). With two patches inserted, we are able to produce a higher attack success rate, with 369 detected examples. After running \tool{} on both our adversarial and clean datasets, we find our TP rate to be 99.19\% and our TN rate to be 95.25\% (see Table \ref{tab:known_attacks_results}). Additionally, we perform an experiment to measure how often \tool{} is able to successfully detect both patches by checking whether the generated masks are disjoint and cover substantial portions of both patches. We find that \tool{} discovers both patches 97.4\% of the time, which we consider to be sufficiently accurate relative to the TP and TN values.

% The accuracy metrics for our multiple patch experiments are slightly higher than our original patch experiments.  One reason for this could be due to a nice property of our CanaryNet framework; the stronger the attack is, the stronger our defense.  CanaryNet begins to fail when clean patches of the images produces similar effects as the adversarial patches, meaning a stronger attack is easier to distinguish using our statistical techniques.  The more important takeaway from this experiment is that our framework is shown to be able to work under a variety of attack conditions without any modifications to our methodology.

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{figures/dummy.png}
% 	\caption{additional plot for non mask reduction}
% 	\label{fig:pull_figure}
% \end{figure}

% \begin{table}[tbp]
% 	\centering
% 	\footnotesize
% 	\begin{tabular}{|c|c|c|c|c|} \hline
% 		--                  & TP    & FP    & TN    & FN    \\ \hline
% 		W.o. Mask Reduction & --    & --    & --    & --    \\
% 		W. Mask Reduction   & 0.997 & 0.003 & 0.970 & 0.030 \\
% 		\hline
% 	\end{tabular}
% 	\caption{Empty table}
% 	\label{tab:performance_results}
% \end{table}

% \begin{table}[tbp]
% 	\centering
% 	\footnotesize
% 	\begin{tabular}{|c|c|c|c|c|} \hline
% 		--                  & TP    & FP    & TN    & FN    \\ \hline
% 		W.o. Mask Reduction & --    & --    & --    & --    \\
% 		W. Mask Reduction   & 0.997 & 0.003 & 0.970 & 0.030 \\
% 		\hline
% 	\end{tabular}
% 	\caption{Runtime table}
% 	\label{tab:performance_results}
% \end{table}

\begin{figure*}
	\centering
	\begin{subfigure}[b]{.19\linewidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/video/clean_000.png}\\
		\vspace{0.12cm}
		\includegraphics[width=1\columnwidth]{figures/video/patch_000.png}
	\end{subfigure}
	\begin{subfigure}[b]{.19\linewidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/video/clean_150.png}\\
		\vspace{0.12cm}
		\includegraphics[width=1\columnwidth]{figures/video/patch_150.png}
	\end{subfigure}
	\begin{subfigure}[b]{.19\linewidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/video/clean_300.png}\\
		\vspace{0.12cm}
		\includegraphics[width=1\columnwidth]{figures/video/patch_300.png}
	\end{subfigure}
	\begin{subfigure}[b]{.19\linewidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/video/clean_450.png}\\
		\vspace{0.12cm}
		\includegraphics[width=1\columnwidth]{figures/video/patch_450.png}
	\end{subfigure}
	\begin{subfigure}[b]{.19\linewidth}
		\centering
		\includegraphics[width=1\columnwidth]{figures/video/clean_600.png}\\
		\vspace{0.12cm}
		\includegraphics[width=1\columnwidth]{figures/video/patch_600.png}
	\end{subfigure}
	\caption{224x224 video frames without (top) and with (bottom) a physical adversarial patch used for our evaluation.}
	\label{fig:physical_atta}
\end{figure*}


\subsection{Runtime Analysis}
\label{sec:performance}

% \begin{table}
% 	%\footnotesize
% 	\centering
% 	\caption{Runtime of Analysis of \tool{}. Wallclock times of each individual component and of the total sequential and parallelized time are shown. Selective search is the only component of \tool{} executed on CPU.}
% 	\begin{tabular}{l r}
% 		\toprule
% 		\textbf{Operation} & \multicolumn{1}{c}{\textbf{Runtime (s)}} \\
% 		\midrule
% 		Selective Search (on CPU)   & 2.3 \\%2.25                                     \\
% 		Forward Pass       & 2.5                                      \\
% 		Class Proposal     & 2.5                                      \\
% 		Grad-CAM           & 0.4 \\%0.35                                     \\
% 		\midrule
% 		\textit{Sequential Total}   & 23.3                                     \\
% 		\textit{Parallelized Total} & 7.7                                      \\
% 		\bottomrule
% 	\end{tabular}
% 	\label{tab:runtime_analysis}
% \end{table}

% Finally, we evaluate the overhead of our defense in terms of rounded wallclock time in Table \ref{tab:runtime_analysis}, using a VGG-16~\cite{simonyan2018vgg16} architecture as a case study.  All components---except for the selective search algorithm---are executed on a Tesla K-80 GPU. Selective search is run on CPU.  In general, a forward pass through the network takes 2.5 seconds, regardless of batch size, while the selective search and Grad-CAM each take 2.25 and 0.35 seconds respectively. If we use a sequential approach to implement \tool{}, we will perform a forward pass to get the initial prediction on input $x$, a selective search on $x$, class proposal on $x$, three Grad-CAMs on the highest class proposals, and three iterations of two batched computations to get $AvgConf$ and $Fooled$ to get a total runtime of 23.3 seconds.  However, many steps can be computed in parallel given enough computational resources.  In general, the original prediction and class proposals can be computed in parallel, as well as the three Grad-CAM computations and the final 6 batched computations.  This cuts the total time down to 7.7 seconds, which is 3x as large as the original prediction time of 2.5 seconds.  We note the wall-clock time is an upper bound value due to overhead introduced by our PyCaffe implementation; a barebone forward pass should be on the order of milliseconds. %\GP{Explain this is an upper bound because of overhead introduced by Caffee when doign a forward pass to the network}

Finally, we measured the latency of \tool{} when protecting a VGG-16~\cite{simonyan2018vgg16} architecture as a case study. All components---except for the selective search algorithm---are executed on a Tesla K-80 GPU. A single execution of \tool{} consists of a run of the selective search algorithm, the Grad-CAM, and a forward pass with a batch of test images. Using the off-the-shelf implementations, the runtime of selective search and Grad-CAM is $2$ and $0.4$ seconds respectively. The forward pass through the network takes about $2.5$ seconds. However, we note that the forward pass runtime is greatly penalized by the overhead introduced by our PyCaffe implementation---a barebone forward pass of the VGG-16 is expected to take from $0.04$ to $0.1$ seconds~\cite{cnn_benchmarks}. With an expected worst-case execution runtime of $0.1$ seconds, and that the forward pass runtime is independent of the batch size, the total latency introduced by \tool{} amounts to $2.5$ seconds.

% Finally, we assess the overhead of \tool{} considering a Titan X multi-GPU system and using a VGG-16~\cite{simonyan2018vgg16} architecture as a case study. The initial forward pass through the network on input $x$ can take in average about $0.04$ seconds~\cite{cnn_benchmarks}, whereas a selective search and class proposal on $x$ take about $2$ seconds~\cite{redmon2016yolo9000} consecutively. As these two steps can be executed in parallel, the total time of the first phase is $2$ seconds. Then, for the mask generation, the Grad-CAM runtime are under-reported in the literature, and we estimated an upper-bound of 0.4 seconds for the execution time of three Grad-CAMs on a less powerful Tesla K-80 GPU. After the mask generation, \tool{} evaluates the network with the generated test images. Given enough computational resources, the runtime of the forward pass is independent of the batch size, taking about $0.04$ seconds~\cite{cnn_benchmarks}. Overall, we estimate that \tool{} takes about 2.5 seconds to determine whether an input is adversarial. 


\section{Adaptive Attacks}
\label{sec:adaptive_attacks}

Our previous analysis demonstrates \tool{}'s versatility in protecting neural networks from a variety of attacks. In this section, we evaluate the more challenging and realistic threat model of a fully adaptive white-box adversary~\cite{carlini2019evaluating} that is aware of the presence of \tool{}, of its architecture and its inner workings. Such an adversary can attempt to create adversarial objects that simultaneously fool the target network while also compromising the core components of \tool{}, i.e., the mask generation, the class proposal, and the attack detection. In \Cref{sec:attacking_region_proposal}, we present attacks aimed at fooling the mask generation phase. Then, in \Cref{sec:attacking_class_proposal}, we evaluate attacks against the class proposal. Finally, in \Cref{sec:attacking_classification}, we present attacks against the attack detection phase.

\subsection{Attacking the Region Proposals}
\label{sec:attacking_region_proposal}

\begin{figure*}[ht]
	\centering
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/dog_patch.png}
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/orig_heatmap.png}
		\caption{Heatmap of the adv. patch}
		\label{fig:dog_patch_1}
	\end{subfigure}~~
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/gradcam_attack_cropped.png}
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/attack_heatmap.png}
		\caption{Full image perturbation}
		\label{fig:dog_patch_2}
	\end{subfigure}~~
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/gradcam_attack_bottom_right_cropped.png}
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/attack_heatmap_bottom_right.png}
		\caption{Localized perturbation}
		\label{fig:dog_patch_3}
	\end{subfigure}~~
	\begin{subfigure}[b]{.24\linewidth}
		\centering
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/gradcam_attack_top_left_cropped.png}
		\includegraphics[width=0.48\linewidth]{adaptive_attack_figs/attack_heatmap_top_left.png}
		\caption{Misdirection}
		\label{fig:dog_patch_4}
	\end{subfigure}
	\caption{Attacking region proposal. \textbf{(a)} The heatmap of the adversarial patch overlaid on an image of a dog. \textbf{(b)} Full-image perturbations can generate a visually identical heatmap. \textbf{(c)} Localized perturbation can generate the same heatmap of (a). \textbf{(d)} Localized perturbation fails to generate a similar  heatmap.}
	\label{fig:dog_patch}
\end{figure*}

Our defense is reliant on successfully localizing the adversarial region in an image. In our current framework, this is done using the Grad-CAM algorithm, which generates a heatmap of the salient regions leading to a classification. If an attacker can disrupt the Grad-CAM mechanism and avoid successful detection and localization, the subsequent components of the pipeline will fail. We observe that the Grad-CAM mechanism uses network back-propagation to measure region importance. As this mechanism is differentiable, an adversary could generate targeted gradient perturbations to control the position and size of the heatmap. In this section, we consider three of these attacks: Grad-CAM perturbation, misdirection of the mask creation, and mask minimization. However, as the analysis of this section shows, while manipulating the heatmap is feasible in theory, in our defense context heatmap manipulation is ineffective in practice.

%\vspace{0.1cm}\noindent\textbf{Perturbing Grad-CAM}---

\subsubsection{Perturbing Grad-CAM}

Consider the adversarial image and its Grad-CAM heatmap in \Cref{fig:dog_patch_1} for the target class ``toaster''. The heatmap in \Cref{fig:dog_patch_1} correctly identifies the area containing the patch. An adversary could try to generate a perturbation, i.e., an adversarial image, resulting in a visually identical heatmap. Such a perturbation can be created in practice as the Grad-CAM function $L^c_{GradCAM} = ReLU(\Sigma_k \alpha_c^{k} A^k)$ is differentiable, and the adversary can optimize an input on this function given a target class. For example, the adversary can use a standard Stochastic Gradient Descent Optimizer (SGD) on a VGG-16 network~\cite{simonyan2018vgg16} to minimize a loss function calculated as the total difference between the current Grad-CAM output and the target Grad-CAM output, and iteratively add noise until the loss converges. An example of such a perturbation is shown in \Cref{fig:dog_patch_2}.

This attack shows that Grad-CAM outputs can be precisely manipulated through gradient optimization. However, such an attack requires to feed the network with a perturbation of the size of the input of the network being protected, which is not part of our threat model (\Cref{sec:threat_model}).

%For example, starting from random noise, which does not have any salient regions for the ``toaster'' class, and optimize the input on our loss function.  We demonstrate in Figure \ref{fig:dog_patch} that the heatmap output of the generated noise at convergence is visually identical to the original heatmap.  This conclusively shows that Grad-CAM outputs can be precisely manipulated through gradient optimization. However, to mount such an attack, the attacker is required to add noise to the entire image, which may not be feasible.



% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/gradcam_attack_cropped.png}
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/attack_heatmap.png}
% 	\caption{object detector}
% 	\label{fig:grad_cam_attack}
% \end{figure}

%\vspace{0.1cm}\noindent\textbf{Heatmap Misdirection}---

\subsubsection{Heatmap Misdirection}

In this attack, we consider an adversary who intends to create an input image that tricks \tool{} to detect the adversarial object in a different region where the adversarial object is located. Let us assume the adversary intends to convince \tool{} that the adversarial object is in the position as indicated by the heatmap of \Cref{fig:dog_patch_1}.
As we demonstrated earlier, an adversary allowed to add perturbational noise to an entire image can generate a heatmap at the desired position. As we discussed before, the adversary does not have full control of the whole image, rendering the attack infeasible. An attacker may try to generate a heatmap visually identical to the adversarial patch of \Cref{fig:dog_patch_1} by using a perturbation constrained to the same region. \Cref{fig:dog_patch_3} shows an example of such a perturbation obtained by modifying the loss function of the SGD to constrain the noise on the same region of interest. At this point, the adversary can try to generate a perturbation at a different location leaving the goal of the attack unchanged. An example of such an attempt is shown in \Cref{fig:dog_patch_4}. The perturbation is now on the top-left corner of the input image. However, the resulting heatmap is not shown in the desired position, i.e., bottom-right. Instead, the heatmap is positioned nearby the location of the perturbation, indicating that localized noise can only affect the corresponding Grad-CAM region.

% A potential behavior an attacker might attempt to generate is heatmap region misdirection, where the heatmap proposes a region that does not cover the adversarial region to either increase the region captured or avoid detection altogether.  We demonstrate earlier that this is trivially possible if the attacker is allowed to add perturbational noise to an entire image.  However, in our setting, the attacker cannot add noise beyond the region of the localized attack, and therefore Grad-CAM perturbations must also be constrained to the adversarial region.  Therefore, the threat we want to consider is that an attacker can add noise in one region of an image that increases the Grad-CAM output value in a disjoint region. We again consider the target heatmap of our adversarial patch in Figure \ref{fig:dog_patch}.  We first show in Figure \ref{fig:dog_patch} that if noise region overlaps the Grad-CAM location we want to modify, we will able to modify the heatmap successfully.  We also show in Figure \ref{fig:dog_patch} that if the noise region is disjoint from the target Grad-CAM region, our Grad-CAM optimization fails to achieve either visual similarity or equivalent final convergence loss.  These experiments show that localized noise can only affect the corresponding Grad-CAM region, which strongly suggests that a misdirection attack is not possible.


% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/gradcam_attack_bottom_right_cropped.png}
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/attack_heatmap_bottom_right.png}
% 	\caption{object detector}
% 	\label{fig:attack_bottom_right}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/gradcam_attack_top_left_cropped.png}
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/attack_heatmap_top_left.png}
% 	\caption{object detector}
% 	\label{fig:attack_top_left}
% \end{figure}

%\vspace{0.1cm}\noindent\textbf{Heatmap Minimization}---

\subsubsection{Heatmap Minimization}

An alternative strategy to fool \tool{} is to minimize the corresponding Grad-CAM region to the greatest extent possible to avoid detection. For example, the adversary can achieve that by modifying the loss function of SGD to optimize for minimal Grad-CAM output. The adversary can start from the adversarial patch image in \Cref{fig:gradcam_minimization} and iteratively add perturbational noise to the region. \Cref{fig:gradcam_minimization}, we show that as our loss converges, the Grad-CAM output is successfully minimized, avoiding detection of the patch.

Our analysis shows that heatmap minimization, i.e., fooling \tool{}, is in tension with the attack success rate of the patch, i.e., fooling $f_m$. \Cref{fig:gradcam_minimization} shows that as more noise is added to the patch, the success rate of the attack is reduced. This result suggests that Grad-CAM is capturing some inherent saliency of the region and cannot be minimized without reducing the attack effectiveness.

The tension between the two objectives could be solved by creating a perturbation that optimizes both for targeted misclassification and for heatmap minimization. Let us consider an adversary that attempts to jointly generate a patch for both criteria by optimizing both objectives during every iteration. Also, to better explore the role played by each objective, we introduce a weighting parameter $\alpha \in [0, 1]$ between the two objectives (i.e., the misclassification objective has weight $\alpha$, and the heatmap minimization has weight $1-\alpha$).
To evaluate then attack, we generate 40 adversarial patches as described by Brown at al.~\cite{brown2017adversarialpatch} for a range of weighting values $\alpha \in [0,1]$. For each patch, we select 100 images from the Imagenet test set~\cite{deng09imagenet} and apply the patch. In total, we generated 4{,}000 malicious images for each weighting ratio $\alpha$. Then, we counted the patches that fool the model, the Grad-CAM\footnote{We use a $<0.5$ overlap ratio between the adversarial pixels and the Grad-CAM region.}, or both.

The results of our experiment are shown in \Cref{fig:joint_adaptive_patches}. As patches work with slight variance, we averaged the attack result to give a better sense of how well a patch would perform. As can be seen in \Cref{fig:joint_adaptive_patches}, there is an inverse relationship between the effectiveness of a patch in fooling $f_m$ (in red) and the region proposal of \tool{} (dashed green), corroborating our previous findings. Additionally, we further plot the patches that successfully fulfill both criteria (in dashed purple), and find that the optimum value is where the ratios of successful misclassifications and hidden patches overlap, giving us patches that fulfill both criteria with an average success rate of 10\%. This strongly suggests that minimizing the Grad-CAM output directly weakens the attack effectiveness and that it is difficult to optimize for both objectives jointly.

%Among all the patches we created, the strongest one managed to fool \tool{} on 31\% of the tested images, at a weighting ratio 0.675. %For comparison, note that on CIFAR10~\cite{cifar10}, an error of ~55\% on $\ell_\infty$ adversarial examples remains the state-of-the-art (see Madry et al.~\cite{madry2018towards}).
%While we acknowledge that this detection accuracy is not perfect, it is worth putting this in perspective with the very strong fully adaptive white-box threat model considered here (where few defenses can claim any increase in robustness), and with potential fault-tolerant deployments of a visual classifier in a practical setting. For instance, in a physical deployment where a neural network is used to classify an incoming stream of images, a successful attack would likely require to reliably and robustly fool the target model on a majority of classified images. In this sense, \tool{}'s detection accuracy may already thwart many attacks.




% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/gradcam_min_attack_bottom_right_10_cropped.png}
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/attack_min_heatmap_bottom_right_10.png}\\
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/num_fooled_plot.png}
% 	\caption{The top row shows a new adversarial patch that can minimize the Grad-CAM output of label ``toaster'' on the location of the patch. However, the bottom plot shows that as the Grad-CAM output sum decreases, the attack success drops correspondingly.}
% 	\label{fig:gradcam_minimization}
% \end{figure}



% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{sentinet_figs/num_fooled_plot.png}
% 	\caption{additional plot for accuracy degradation}
% 	\label{fig:accuracy_degradation_plot}
% \end{figure}

% However, we would also expect the effectiveness of the attack to drop with the addition of any arbitrary noise, and does not rule out the possibility of perturbational noise that can optimize both targeted misclassification and Grad-CAM minimization. Our next experiments demonstrate how an attacker might attempt to jointly generate a patch for both criteria by performing both optimization functions during every iteration. We use a range of $\alpha$ from 4.0 to 1.0 with intervals of 0.025 and set the learning rates of the Grad-CAM minimization and the misclassification as $(\alpha)$  and $(1 - \alpha)$ respectively, as seen in Figure \ref{fig:joint_adaptive_patches}. This adjusts the level or prioritization we set for each optimization task.  After we generate 40 patches for each $\alpha$ value, we plot the average of both the percentage of successful misclassifications on Imagenet~\cite{deng09imagenet} test set $X$ from Attack \#3 and the percentage of patches with $<0.5$ overlap with the adversarial pixels and the Grad-CAM region in Figure \ref{fig:joint_adaptive_patches}.  Our plot shows that there is an inverse relation between how well the patch fools test images and how well the patch is hidden, corroborating our previous findings.  We further plot the patches that successfully fulfill both criteria in Figure \ref{fig:joint_adaptive_patches}, and find that the optimum value is where the ratios of successful misclassifications and hidden patches overlaps, giving us patches that fulfill both criteria at most a 10\% success rate.  This strongly suggests that minimizing the Grad-CAM output directly weakens the attack effectiveness, and that it is difficult to jointly optimize for both objectives.

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/adaptive_adversarial_0_patch.jpg}
% 	\includegraphics[width=0.4\columnwidth]{adaptive_attack_figs/adaptive_adversarial_1_patch.jpg} \\
% 	\includegraphics[width=0.8\columnwidth]{adaptive_attack_figs/merged.png}
% 	\caption{In the top row, the left and right patches are generated to maximize Grad-CAM minimization and Attack success respectively.  We can see in the bottom row plot that it is difficult to optimize for both objectives, and that patches that successfully fulfill both objectives can achieve at most 10\% effectiveness in both bypassing Grad-CAM and attacking successfully.}
% 	\label{fig:joint_adaptive_patches}
% \end{figure}

% \begin{figure}[!htbp]
% 	\centering
% 	\includegraphics[width=0.8\columnwidth]{adaptive_attack_figs/merged.png}
% 	\caption{object detector}
% 	\label{fig:joint_adaptive_plot}
% \end{figure}

\begin{figure}[htb]
	\centering
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=0.44\columnwidth]{adaptive_attack_figs/gradcam_min_attack_bottom_right_10_cropped.png}
		\includegraphics[width=0.44\columnwidth]{adaptive_attack_figs/attack_min_heatmap_bottom_right_10.png}\\
		\includegraphics[width=1\columnwidth]{sentinet_figs/num_fooled_plot.png}
		\caption{Heatmap minimization}
		\label{fig:gradcam_minimization}
	\end{subfigure}
	\begin{subfigure}[b]{.49\linewidth}
		\centering
		\includegraphics[width=0.44\columnwidth]{adaptive_attack_figs/adaptive_adversarial_0_patch.jpg}
		\includegraphics[width=0.44\columnwidth]{adaptive_attack_figs/adaptive_adversarial_1_patch.jpg} \\
		\includegraphics[width=1\columnwidth]{adaptive_attack_figs/merged.png}
		\caption{Minimization and attack}
		\label{fig:joint_adaptive_patches}
	\end{subfigure}
	\caption{Heatmap minimization attack. \textbf{(a)} Example of adversarial input minimizing the Grad-CAM output (top); Plot showing the tension between minimization and attack success. \textbf{(b)} Patches minimizing the heatmap and maximizing the attack success respectively (top); Plot of success of the patch vs. minimization of the heatmap.}
\end{figure}

%\vspace{0.1cm}\noindent\textbf{Results}---

\subsubsection{Results on Attacking Region Proposals}

To summarize, in this section, we presented three attacks against the Grad-CAM algorithm. Our evaluation shows that, while the Grad-CAM output can be perturbed with localized perturbations, misredirecting the Grad-CAM heatmap seems an infeasible attack strategy. Also, our results show that minimizing the heatmap size dramatically reduces the effectiveness of the attack. Accordingly, we conclude that attacking the Grad-CAM algorithm may bring a very little advantage to an adversary.


\subsection{Attacking the Class Proposal}
\label{sec:attacking_class_proposal}

Another approach to avoid the localization of the adversarial region is attacking the class proposal step. In this section, we discuss attacks exploiting the algorithms implemented in the class proposal step. In particular, we concentrate on two types of attacks where the adversary intends avoiding detection by generating masks without the adversarial region or weakening the detection by creating inefficient masks.

%\subsubsection{Avoiding Detection with Weak Primary Class Prediction} The goal of the first attack intends avoiding the detection of the target class. Here, the adversary may create a patch for a target class that is not identified as the primary class, i.e., the first class identified by the class proposal step. With such an attack, \tool{} will create a mask for the primary class that will not include the patch, effectively bypassing \tool{}. However, such an attack is very unlikely to take place because the final prediction of the model is the primary class, i.e., $y=f_{m}(x)$ where $x$ is the input image. %Accordingly, it very unlikely that an adversary may choose avoiding detection by attacking the proposal of the primary class.

\subsubsection{Mask Reduction with Specialized Patch Sub-regions} Instead of avoiding detection, the adversary may try to weaken the detection of the patch by reducing the size of the mask of the primary class. The goal of the class proposal is to identify additional classes in the input image to remove ambiguous areas (see \Cref{fig:precise_mask}a-b). Here, the attacker may try tricking the class proposal into identifying classes in sub-regions of the patch. Such an attack results in a mask containing only a portion of the entire patch, thus weakening the response of the model at test time and the detection of the attack.

The creation of a localized universal patch exposing such behavior may be very challenging. Such a patch needs to have a region causing the activation of a class, say $y'$, and, at the same time, another region for the target class $y$. Also, to carry this attack, the patch should cause a change in the prediction of the model when the region for $y'$ is missing. Building a localized universal patch with such a non-linear dependency between the two regions may be hard, if not unfeasible, and we hope other researchers will explore whether such a type of attack is possible.

\subsubsection{Avoiding Mask Reduction by Over-Segmentation} Mask reduction removes from the primary mask areas that are ambiguous, resulting in more efficient masks. Instead of generating inefficient mask by removing malicious regions, the adversary may try to bypass the mask reduction and generate large, ineffective masks like the one shown in \Cref{fig:precise_mask}a. To achieve such a goal, the adversary might attack the image segmentation algorithm, i.e., selective search~\cite{uijlings2013selectivesearch}, and trick the algorithm into returning many small segments outside of the malicious region. When processing small segments, the network may return predictions with low confidence which are ignored when generating the mask for the primary class (see \TopConf{$C$, $k$} in \Cref{alg:class_proposal}). As a result, the final mask will not be refined by removing the ambiguous areas thus weakening the response of the model at test time.

However, attacking the selective search algorithm may not be a feasible strategy. Our inspection of the selective search algorithm revealed that an adversary controlling a limited region of the input image may not be able to influence the generation of a segment of arbitrary size and position. As a result, we believe that attacking the selective search algorithm may be unlikely.


% The first step of \tool{} consists of proposing a list of classes present in the input $x$. Our class proposal module relies on selective search~\cite{uijlings2013selectivesearch}, a traditional graph-based image processing algorithm, to exhaustively segment an image based on color, shapes, textures, and size. Then, the class proposal module uses the network under protection with a ROI pooling layer to predict the class of each segment~\cite{girshick2015fastrcnn}. 

% As the selective search is not based on gradients, an adversary cannot rely on perturbations to hijack the segmentation phase. Our selective search algorithm is also designed to capture class proposals other than adversarial class, and the attacker will be unable to affect the selective search results outside of the adversarial region.  Furthermore, because our proposal network uses the original network weights, there is no way to cause different behaviors between the original and proposal networks. Finally, the attacker will have limited motivation to attack the class proposal process of our network, as a successful attack will damage the accuracy of the attack detection rather than break the entire process. In conclusion, our analysis indicates that our class proposal mechanism is robust due to the properties of the individual components that are collectively resistant to perturbational attacks.

% \GP{Can you add some introductory text here and leave the description of the attack in the Attack \#8 part?}

% \vspace{0.1cm}\noindent\textbf{Attack \#8: Class Proposal}---Our class proposal module uses selective search and a proposal network modified from the original network with a ROI pooling layer.  Selective search is a traditional image processing algorithm that uses a graph-based approach to segment an image based on color, shapes, textures, and size. There is no gradient component for an attacker to perturb, or a training procedure to poison, which severely limits an attacker's mechanisms of attack compared to a network-generated proposal mechanism as seen in Faster-RCNN.  Our selective search algorithm is also designed to capture class proposals other than adversarial class, and the attacker will be unable to affect the selective search results outside of the adversarial region.  Furthermore, because our proposal network uses the original network weights, there is no way to cause different behaviors between the original and proposal networks. Finally, the attacker will have limited motivation to attack the class proposal process of our network, as a successful attack will damage the accuracy of the attack detection rather than break the entire process.  We can conclude that our class proposal mechanism is robust due to the properties of the individual components that are collectively resistant to perturbational or poisoning attacks.

\subsubsection{Results on Attacking the Class Proposals}

To summarize, in this section, we presented three attacks against the algorithms that propose a list of classes present in the image $x$. Our evaluation shows that the goal of avoiding the prediction of the primary class conflicts the goal to hijack the final prediction. Also, our analysis suggests that creating inefficient masks may be either remarkably challenging---if not infeasible---or even not possible. Accordingly, we conclude that attacking the class proposal step may bring little to no advantages to an adaptive adversary.

\subsection{Attacking the Attack Classification}
\label{sec:attacking_classification}
% \GP{Same as before: add some}

We now consider attacks aimed at fooling the decision procedure of \tool{}.
%\vspace{0.1cm}\noindent\textbf{Classification}---
%\subsubsection{Classification}

We now consider attacks aimed at fooling the decision procedure of SentiNet, where extracted regions or inert patterns are overlaid onto benign test images to measure their generalizability. One possible attack in the context of poisoned or trojaned networks has the adversary manipulate the model so that it recognizes the inert pattern as a member of a targeted class. This would let the attacker bypass our defense as adversarial patterns will remain adversarial when overlaid with the``inert'' pattern. This attack does not apply to the setting where an adversary aims to evade an uncompromised network with adversarial patches. For the general case, we note that the choice of inert pattern can be made after the network has been trained, so one can test whether the chosen pattern affects the model. We also found that using patterns made up of various random patterns or noise (see~\Cref{fig:secret_patterns}) produce good results, which further hinders a training-time adversary’s ability to target the specific pattern than will later be used at test-time.
For example, in \Cref{tab:known_attacks_results}, we can see that for the evaluation with the trojaned network, the TP and TN rates of the random noise pattern and checker pattern are within $\leq 0.25\%$.

% \GP{Should?! This is hand-waving and it seems we are not well covered here. What else can we say? Would it be possible to create an inert patch with gradient descent? Instead of maximizing can we minimize the response of all classes... would this work?}

% \subsubsection{Summary}\GP{It is weird to have a summary with additional attacks. I would create a own category for these and then have a summary. Perhaps, instead of having a summary for the adaptive attacks, I would propose a Summary subsection to summarize the entire section. A sort of takeaway for the entire evaluation. I would like to see sentences glorifying the good qualities/properties of \tool{}}

% We have shown empirically or through design choices that the region proposal (1), the class proposal (2), and the attack classification (3) portions of our attack are individually robust to attacks.  We also propose and discuss several other adaptive attacks that can bypass our defense mechanism.

%\GP{We have this already}

%\vspace{0.1cm}\noindent\textbf{Attack \#9: Patterns Targeting Different Classes}---

%\vspace{0.1cm}\noindent\textbf{Attack \#10: Size Attack}---

% \subsubsection{Size Attack}

% Our focus with \tool{} is to capture adversarial attacks that are unreasonably salient, designed to be small and unnoticeable. With this measure, \tool{} largely succeeds at detecting abnormal regions of images that deviate from patches of natural images. When adversaries can modify the majority of pixels in an image, they can override the prediction. As noted by Brown et al.~\cite{brown2017adversarialpatch}, large images of an actual toaster will hijack the same prediction of an adversarial patch at a large enough size, raising the interesting question about what actually constitutes an ``attack''. Based on this observation, we note that the attack's $avgConf$ drops as the size of the object increases, and by increasing the transparency of the object, the attack drops below the threshold while retaining very high attack success (See \Cref{fig:size_analysis}). Similarly as observed by Brown et al.~\cite{brown2017adversarialpatch}, drop of $avgConf$ and high attack success is the result of obfuscating the test inputs with the large targeted class. As a result, we conclude that our defense correctly captures small patches and we defer to future work addressing the challenge of unreasonably large objects.


% If the attacker uses a large enough patch, the average confidence on $X$ will be lowered, which reduces the effectiveness of our defense.  We can see in \Cref{fig:size_analysis} that for adversarial patches, the attack's $avgConf$ drops as the size of the patch increases.  By increasing the transparency of the patch, we can drop the attack below the threshold while retaining very high attack success.  However, we argue that this is an unavoidable aspect of localized attacks.  Brown et al.~\cite{brown2017adversarialpatch} note that overlaying an image of an actual toaster will create the same behavior of an adversarial patch at a large enough size.  This raises interesting questions about what actually constitutes an ``attack'', although for now, we can conclude our defense captures small patches that abnormally affect the classification results at an extent greater than expected for natural images.






% \subsection{Takeaway}
% In Attacks \#1-4, we show that \tool{} is highly generalizable and detects adversarial inputs with high TP and TN results across a variety of different attack mechanisms and shapes without modification between experiments.  In Attacks \#5-8, we examine a variety of techniques an adaptive adversary can consider and show why they are difficult to implement, demonstrating the individual components of \tool{} are robust.  In Attack \#9, we do show that large patches can defeat our mechanism, but what these results mean will be discussed in Section \ref{sec:limitations}. We also calculate the runtime to give a general sense of the overhead \tool{} introduces.

% \GP{here, we can distill the list of goals achieved and the good things our experiment showed up. Keep this discussion factual on the experiments. For example, "We can detect this this and this attack", "we showed that an adaptive adversaries has little manouver", and "however, extremely large patches can defeat our mechanisms". What these results entail or mean will be part of Section "Discussion".}

==> Archive 2/introduction.tex <==
% !TeX root = ./main.tex
\section{Introduction}

% Deep learning has gained importance in our daily life due to its tremendous success in various tasks such as image and speech recognition~\cite{zhang2018dlreview}. Deep learning systems are use neural networks with millions of neurons requiring a training over millions of data items. As the complexity of neural networks is increasing, training a custom neural network is no longer a viable option. As a result, developers tend to reuse existing pre-trained, existing neural networks for the new task.

% \GP{The intro should focus on the actual security threats: 1) using models susceptible to adverversarial attacks and 2) re-using compromised models.}

Deep neural networks are susceptible to a variety of attacks aimed at causing misclassifications~\cite{szegedy2013boxlbfgs,goodfellow2014fgsm, brown2017adversarialpatch}.
As deep learning models are also often re-used (e.g., via transfer learning~\cite{bengio2012deep}), model vulnerabilities---whether inherent or purposefully inserted by a malicious party~\cite{Liu2018TrojaningAO}---can easily affect a large number of systems.
This has severe implications for the trustworthiness of deep learning models in security-critical decision-making situations.
Defending against these attacks is challenging due to the wide variety of possible attack mechanisms and vectors, especially for models operating in the visual domain. In this work, we explore \emph{localized} and \emph{universal} attacks on visual classifiers and introduce \tool{}, a robust defense which detects adversarial inputs without requiring any specific model re-training or prior knowledge of the attack vector.

We focus on attacks that are \emph{localized}, i.e., the adversarial region is constrained to a small contiguous portion of an image, and \emph{universal}, i.e., attacks are image-agnostic. 
Inputs with these properties have proven useful for instantiating robust and physically realizable attacks that take the form of an adversarial object or sticker placed inside a visual scene~\cite{brown2017adversarialpatch, Liu2018TrojaningAO,evtimov2017robust,eykholt2018physical}. These classes of attacks typically use \emph{unbounded} perturbations (i.e., without any specific $\ell_\infty$ or $\ell_2$ constraint as in most digital attacks~\cite{szegedy2013boxlbfgs, goodfellow2014fgsm}), to ensure that the attacks are robust to changes in viewpoint, lighting and other physical artifacts. 
Several such physical attacks have been demonstrated, with the goal of causing misclassifications when applied to arbitrary images with different class labels~\cite{brown2017adversarialpatch, Liu2018TrojaningAO}.
A drawback of localized attacks is that they are generally visible and detectable by the human eye, but there are many situations where attacks can be deployed in autonomous settings or carefully disguised~\cite{brown2017adversarialpatch}.


% A wide variety of attack and deployment mechanisms have been used to create localized physical attacks.
% This makes the defender's task very difficult, as attack-specific defenses must be combined together for comprehensive security. 
A prospective defender must first consider that the model being protected may have been compromised prior to being deployed.
% It is common in the deep learning setting to share and use pre-trained networks; for example to fine-tune a traffic-sign recognition network~\cite{gu2017badnets}.
An attack can originate from the source of the network provider, as in the case with data poisoning attacks~\cite{gu2017badnets}, or can be intercepted and modified, as with trojaning attacks~\cite{Liu2018TrojaningAO}.
% This means the defense potentially needs to be specifically tailored for each pretrained model to protect against attacks that will only affect that particular model.
Even if a network is integrity protected, adversaries can still generate localized and universal attacks that will affect the model at test time, via adversarial examples~\cite{brown2017adversarialpatch}.
%Furthermore, there are countless permutations positioning and behaviors these attacks could exhibit, all which are unknown to the defense.
% Finally, modifying the network is not a reliable way to prevent misclassifications, and could cause undesirable drops in performance.
Altogether, this creates an extremely difficult security setting where vulnerabilities are easily distributed, where adversaries target properties inherent to neural network systems that cannot be removed, and where attacks might be too diverse in appearance for a signature-based scheme.

Our goal is to create a defense against localized universal attacks that is attack-vector agnostic.
%In a setting where there are countless varieties of models and attacks, we infer that the generalizability of a defense is equivalent to the robustness of the defense.
To this end, we identify unifying and necessary features of successful localized universal attacks---including physically realizable attacks---and develop \tool{}, a novel technique that exploits these attack behaviors to detect them.
We start from the observation that localized universal attacks are designed to be robust to a variety of artifacts while generalizing to a large distribution of inputs (e.g., the adversarial patch of~\cite{brown2017adversarialpatch} is designed to work when applied to \emph{any} input image). 
Our first insight is that a localized universal attacks' success relies on the use of ``salient'' features that strongly affect the model's classification on many different inputs. We thus consider techniques from \emph{model interpretability} and \emph{object detection} to discover highly salient contiguous regions of an input image. As we show, these techniques uncover adversarial image regions, as well as benign ones that strongly affect classification. In a second step, we exploit the strong robustness and generalization properties of malicious regions to distinguish them from benign regions with high saliency. Specifically, we overlay extracted regions on a large number of held-out clean images and test how often this results in a misclassification. Malicious regions are much more likely than benign regions to generate misclassifications and are thus detected by \tool{}. As we show in our evaluation of \tool{}, mounting an attack that evades detection requires lowering an adversarial region's saliency to a point where the region is no longer universal (i.e., it fails with high probability on random inputs)---even for a adaptive adversary with knowledge of \tool{}'s architecture. We also validate \tool{}'s effectiveness in a realistic physical setting, where it successfully detects a printed adversarial patch~\cite{brown2017adversarialpatch} with high reliability.

\paragraph{Contributions} To summarize, this paper makes the following contributions:

% \begin{itemize}
% \item We propose \tool{}, a new architecture that protects a neural network by using the same model to detect physical attacks.  
% \item \tool{} uses a novel approach to detect a potential attack region using techniques developed for model visualization and object detection, and feeds the attack deployed on multiple test images back on the network to perform the attack classification.  
% \item Our architecture is attack agnostic and can defend from distinct families of physical attacks without previously seeing or having knowledge of the attack. 
% \item In one attack setting, we show that we can detect attacks with a true positive rate of 0.991848, a false positive of 0.0025, a true negative rate of 0.997500 , and a false negative rate of 0.008152.
% \item \tool{} can detect attacks in real-time introducing an 3x overhead of 5.35 seconds.
% \end{itemize}

\begin{itemize}
	\item We propose \tool{}, a new architecture that protects a neural network by using the same model to detect localized universal attacks.

	\item To the best of our knowledge, \tool{} is the first architecture that does not rely on prior knowledge of the specific attack vector used to carry the attack, e.g., trojaned networks, poisoned networks, and adversarial patches---including physically realizable attacks.

	\item \tool{} uses a novel approach to detect a potential attack region using techniques developed for model visualization and object detection and feeds the attack deployed on multiple test images back to the network to perform attack classification.
	
	\item We evaluate \tool{} to protect pre-existing compromised and uncompromised networks against three known attack vectors, i.e., backdoors for poisoned networks, triggers for trojaned networks, and adversarial patches for uncompromised networks. We show that \tool{} can protect neural networks successfully, with an average true positive rate of 96.22\% and an average true negative rate of 95.36\%.%\GP{Beef up results: Say whether and when our numbers are above or at the bar of the state of the art. If at the bar, we need to strenthen that we are attack-agnostic.}

	\item We further evaluate \tool{} against a fully adaptive white-box adversary and present seven attacks against \tool{}'s core components. We show that \tool{} is resistant against strong adversaries by demonstrating the robustness of each individual component.

   %\item \tool{} requires no special training and can be instantiated with off-the-shelf neural networks while introducing 2.5s latency at inference time.

\end{itemize}

\paragraph{Paper Organization} In \Cref{sec:background}, we present the architecture of deep learning systems and \tool{}'s threat model. Then, in \Cref{sec:sentinet}, we present \tool{} and its architecture. In \Cref{sec:evaluation}, we evaluate \tool{} against localized universal attacks taken from the literature, as well as against physically printed adversarial patches. In \Cref{sec:adaptive_attacks}, we assess \tool{} against adaptive attackers trying to fool \tool{}'s internal components. Next, in \Cref{sec:discussion}, we discuss our results. Finally, in \Cref{sec:related_work}, we cover related works, and in \Cref{sec:conclusion}, we provide our conclusions.

% \GP{Overview of the structure of the paper. Do empasize the evaluation: three attacks and adaptive attacker.}


==> Archive 2/related.tex <==
% !TeX root = ./main.tex
\section{Related Work}
\label{sec:related_work}

We now review works closely related to this paper. First, we explore the domain of attacks against neural networks. Then, we expand on prior works on localized universal attacks. Finally, we review proposed approaches to detect attacks against neural networks.

\paragraph{Neural Network Attacks} The literature on attacks on neural networks is vast and still growing.  
Szegedy et al.~\cite{szegedy2013boxlbfgs} first demonstrated how adversarial noise can be used to fool neural network classifiers by adding small gradient perturbations to an image that is imperceptible to humans.
Numerous works have built on this approach; some notable works include the Fast Gradient Sign Method~\cite{goodfellow2014fgsm}, DeepFool~\cite{moosavidezfooli2015deepfool}, and Universal Adversarial Perturbations~\cite{moosavidezfooli2016universal}.  
This area of research can be categorized as a cat-and-mouse game in recent years, where defenses are created for new attacks that bypass previous defenses~\cite{carlini2018eval}~\cite{carlini2017tendetection}. Additionally,  attacks certainly are not limited to gradient-perturbation based techniques; data poisoning can be used to cause misintended model behaviors~\cite{shafahi2018poisonfrog}, and compromised hardware can also be used to insert trojans during the network inference procedure~\cite{clements2018hardwaretrojans}.
Akhtar et al.~\cite{akhtar2018adversarialsurvey} provides a useful survey about the current state of the adversarial deep learning field.

\paragraph{Localized Universal Attacks} Multiple works have demonstrated attacks within a variety of classification settings and attacker capabilities. Adversarial patches~\cite{brown2017adversarialpatch} are possibly the most well-known localized universal attack.  These attacks are generated by performing back-propagation on the target class to calculate gradient noise localized to a region of the image. A related attack---Localized and Visible Adversarial Noise~\cite{karmon2018lavan}---operates under a similar principle with smaller but less robust attacks.  Robust Physical-World Attacks on Deep Learning Models~\cite{evtimov2017robust} demonstrates how adversarial perturbations can be disguised as graffiti stickers to fool traffic sign attacks.  Similarly, Sharif et al.~\cite{sharif2016glasses} use perturbations placed on glasses to fool facial classification models.  Trojaned Neural Networks~\cite{Liu2018TrojaningAO} perform back-propagation on specifically chosen neurons in the network rather than the target class. The generated triggers are used to "trojan" the model by performing slight fine-tuning to guide the trigger outputs towards a specified class, making sure that the triggers only cause misclassifications on trojaned models. BadNets~\cite{gu2017badnets} targets traffic sign detection models by inserting pre-chosen patterns into images with the target label, poisoning the data before the training process. 


%%%%% Other Detection Methods
\paragraph{Adversarial Attack Detection} Detection techniques for attacks as a defensive measure have been proposed by many researchers. Safetynets~\cite{lu2017safetynet} is designed to detect adversarial-noise based attacks and exploits the different activations adversarial perturbations produce to train a SVM classifier. Metzen et al.~\cite{metzen2017detectingperturb} use a similar approach by training a modified target classification network to detect adversarial perturbations. Feinman et al.~\cite{feinman2017artifacts} also trains a classifier to detect adversarial perturbational inputs based on the neural network features, while Gong et al.~\cite{gong2017nottwins} introduces a classifier trained to detect adversarially-perturbed images. Magnet~\cite{meng2017magnet} trains a classifier on manifolds of normal examples to detect adversarial perturbations without prior knowledge of the attack. There are also some works designed at creating defenses that do not require training. Grosse et al.~\cite{grosse2017statisticaldetection} uses statistical techniques to distinguish adversarial-perturbations outputs, while Hendrycks et al.~\cite{hendrycks2016earlydetect} uses PCA to visualize differences in perturbed images. A survey by Yuan et al.~\cite{yuan2017attacksanddefenses} covers further detection defenses. All these works are only aimed at defending against adversarial perturbations whereas \tool{} can defend a network against other types of attacks, i.e., data poisoning and trojaning attacks. 

% \vspace{0.2cm}\noindent\textbf{Detection of Occluded Objects}---\GP{Review and discuss the similarity/differences between \tool{} and detection of occluded objects: Detecting Semantic Parts on Partially Occluded Objects (\url{https://arxiv.org/pdf/1707.07819.pdf}), Face recognition with occlusion (\url{https://ieeexplore.ieee.org/document/7486587}), and Recovering Occlusion Boundaries from a Single Image (\url{https://www.ri.cmu.edu/pub_files/pub4/hoiem_derek_2007_3/hoiem_derek_2007_3.pdf})}

% \subsection{Network Visualization}
% There has been interest amongst deep learning practioners in understanding and visualizing neural network behaviors. Yosinski et al~\cite{yosinski2015deepvis} demonstrates a technique to generate saliency maps, which visualize which pixels are most salient towards a particular prediction. Zhou et al.~\cite{zhou2015cam} introduces class activation mapping to create a heatmap regarding the importance of the image regions by modifying and retraining the pooling layer of a neural network. Grad-CAM~\cite{selvaraju2016gradcam} introduces a different technique to perform activation mapping that utilizes the gradients without modifying the original netowrk.
% Grad-CAM++~\cite{chattopadhyay2017gradcamplus} builds on that work further by including pixel-wise weighting for better visualizations.

% \subsection{Object Detectors and Segmentation}
% Object detection and segmentation is a related area where neural networks are used separate and classify regions of an image.
% A family of detection networks, RCNN~\cite{girshick2013rcnn}, Fast-RCNN~\cite{girshick2015fastrcnn}, Faster-RCNN~\cite{ren2015fasterrcnn}, and Mask-RCNN~\cite{he2017maskrcnn}, is based on the approach of producing region proposals and feeding it through a CNN classifier.
% YOLO~\cite{redmon2015yolo} and YOLOv2~\cite{redmon2016yolo9000} represent a separate family of object detection networks that are designed for more efficient but less fine-grained object detection. 
% A third class of networks are trained to perform segmentation on images by using an encoder and decoder structure; several well known networks include FCN~\cite{long2014fcn}, Segnet~\cite{badrinarayanan2015segnet}, and U-Net~\cite{ronneberger2015unet}.

%%%%% Anomaly Detection

==> adaptive_attack.tex <==
Adaptive Attacks:
A considerable number of defenses against adversarial attacks have been proposed only to be broken (cite) by 'adaptive attacks' that adapt to the presence of known defenses.  This has led to a cat-and-mouse game where defenses have to first discover and then account for new attacks constantly being introduced, creating an environment highly advantageous to adversaries.  Our proposed method diverges from this arms race by creating a generalizable defense that does not take the mechanism of an attack, which alleviates the need to tailor-design defenses towards specific attacks and provides the capability of detecting attacks that have not been seen before. We want to explore how robust our method is against adaptive attacks by attempting to compromise each component of our defense.



Threat Model:
	1. Localized universal adversarial patch
		a. Our threat model deals with over-the-air attacks, where you can't just attack a digital image
		b. A sufficiently large image can override any image, as described in "Adversarial Patches" - must be small
		c. Attacks are generally 'universal' - attacks cannot be specific to a specific image in an over-the-air setting, must be robust to viewpoint, resolution, and brightness changes
	2. Our defense assumes - attacks are small, and attacks misguide towards a certain class
		a. Our defense uses GradCam+FRCNN to segment out the small patch
		b. Overlays suspected attack onto other test set I' to get number of misguided (2) and also overlays noise onto test set l' to get the confidence value after noising (1)
		c. Normal images either have high (1) and low (2) (associated with small patches), high (2) and low (1) (associated with large patches), or low (1) and low (2) (large patches of useless information).  Only adversarial images will have high (1) and low (1).
		
	3. Proposed Attack - Thresholding
		a. We do not share I' with any outside parties, which means the attacker cannot manipulate the behavior on I' for either (1) or (2).  The attacker cannot attack the thresholding behavior.
	4. Proposed Attack - Fast RCNN
		a. Fast RCNN consists of two parts - the original network and selective search
		b. Overall, Fast RCNN is used to narrow down our GradCAM mask, so attacking it will only slighly decrease the accuracy of our defense rather than subveting it.
		c. Because we use the original network for classification, if our original network is susceptible, the network used for RCNN will also be susceptible; therefore it is impossible to bypass the bounding box classification network.
		d. Attacking selective search is very difficult due to the exhaustive properties of selective search - selective search is not a gradient descent based technique meaning its hard to construct an adversarial attack; it is based detecting edges and color changes to create many object proposals. Therefore, it is impossible to prevent the bounding boxes from being proposed outside of the patch
	5. Proposed Attack - Multiple Patches
		a. First Attack - disjoint attacks targeting same classes -  our experiment shows this doesn't work
		b. Second Attack - single patch targeting different classes - detect patch + object as the natural object will bypass the FastRCNN eliminations - if more than 3 objects in the same area - reject 
		c. Third Attack -detect patch+object as 1 object - lots of disjoint attacks will bypass the FastRCNN eliminations; we can increase the number of FastRCNN proposals, increasing by linear runtime. 
	6. Proposed Attack - GradCAM
		a. A possible subversion for GradCAM is to make the GradCam activate outside of the patch, either making the mask segment too much of the image out or to miss detecting the patch altogether.  Our experiments show that it is possible to perturb an entire image to create a certain GradCAM output, but it is impossible to affect the GradCAM outputs outside of a localized patch
Another possible attack is to minimize the amount the patch shows up on GradCAM.  We first show that adding perturbed noise to minimize the patch will decrease the effectiveness of the attack.  We show that this is the case even with joint training (show the curve).  We believe this is evidence that that it is impossible to optimize for both minimizing GradCAM and the attack behavior
